Gravitational Waves and Black Holes: an Introduction to General Relativity

In these lectures general relativity is outlined as the classical field theory of gravity, emphasizing physical phenomena rather than mathematical formalism. Dynamical solutions representing traveling waves as well as stationary fields like those of black holes are discussed. Their properties are investigated by studying the geodesic structure of the corresponding space-times, as representing the motion of point-like test particles. The interaction between gravitational, electro-magnetic and scalar fields is also considered.

==> ch1.tex <==
\chapter{Gravity and Geometry}{\label{C1}}

\section{The gravitational force}{\label{S1.1}}

Gravity is the most universal force in nature. As far as we can tell from 
observations and experiments every object, every particle in the universe 
attracts any other one by a force proportional to its mass. For slow moving 
bodies at large distances this is a central force, inversely proportional 
to the square of the distance. As the action is reciprocal, and since 
according to Newton action and reaction forces are equal in magnitude, the 
expression for the gravitational force between two objects of mass $M_1$ 
and $M_2$ at a distance $R$ is then determined to have the unique form

\be
F\, =\, G\, \frac{M_1 M_2}{R^2}.
\label{1.1}
\ee

\nit
The constant of proportionality, Newton's constant of gravity, has dimensions
of acceleration per unit of mass times an area. Therefore its numerical value 
obviously depends on the choice of units. In the MKS system this is

\be
G\, =\, 6.672\,59 (85) \times 10^{-11}\, \mbox{m$^3$ kg$^{-1}$ s$^{-2}$}.
\label{1.2}
\ee

\nit
It is also possible, and sometimes convenient, to fix the unit of mass in such 
a way that Newtons constant has the numerical value $G = 1$. In the natural 
system of units, in which also the velocity of light and Planck's constant are 
unity: $c = \hbar = 1$, this unit of mass is the Planck mass $m_P$:

\be
\ba{lll}
m_P\, =\, \dsp{ \sqrt{\hbar c / G} } & = & 2.176\,71 \times 10^{-8}\, \mbox{kg}\\
  &  & \\
  & = & 1.221\,047 \times 10^{19} \mbox{GeV}/c^2.
\ea
\label{1.3}
\ee
 
\nit
Newton's law of gravity (\ref{1.1}) is valid for any two massive bodies, as 
long as they are far apart and do not move too fast with respect to one 
another. In particular, it describes the motions of celestial bodies like 
the moon circling the earth, or the planets orbiting the sun, as well 
as those of terrestrial objects like apples falling from a tree, or canon 
balls in free flight. Ever since Newton this unification of celestial and 
terrestial mechanics has continued to impress people and has had a tremendous 
impact on our view of the universe. It is the origin and basis for the belief 
in the general validity of physical laws independent of time and place. 

\section{Fields}{\label{S1.2}}

Although as a force gravity is universal, Newton's law (\ref{1.1}) itself
has only limited validity. Like Coulomb's law for the electrostatic force 
between two fixed charges, Newton's law holds strictly speaking only for 
static forces between bodies at rest. Moreover, and unlike the electric 
forces, there are modifications at smaller, finite distances which can be 
observed experimentally.

For example, if the gravitational force would have a pure $1/R^2$ dependence, 
the orbits of particles around a very heavy central body would be conic 
sections: ellipses, parabola's or hyperbola's, depending on the energy and 
angular momentum, in accordance with Kepler's laws. The observation of an 
excess in the precession of the perihelion of the orbit of Mercury around 
the sun by LeVerrier in 1845, and improved by Newcomb in 1882 \ct{SC}, was 
one of the first clear indications that this is actually not the case, and 
that the gravitational force is more complicated.   

The exact form of the gravitational forces exerted by moving bodies is a 
problem with many similarities to the analogous problem in electrodynamics. 
The understanding of electrodynamical phenomena greatly improved with the 
introduction of the concept of local field of force. This concept refers to
the following characteristics of electrodynamical forces:
\begin{itemize} 
\item{ the influence of electric charges and currents, and of magnetic poles, 
extends throughout empty space;}
\item{ the force on a standard test charge or test magnet at any given time 
depends on its location with respect to the source of the field and the 
relative state of motion;}
\item{ changes in the sources of the fields give rise to changes in the force 
on test objects at a later time, depending on the distance; the speed of
propagation of disturbances in empty space is finite.}
\end{itemize}
In the case of electrodynamics this speed turned out to be a universal 
constant, the speed of light $c$. One of the most striking consequences of 
these properties, which follow directly from the mathematical description of 
the fields as expressed by Maxwell's equations, is the existence of 
electromagnetic waves, local variations in the fields which transport energy, 
momentum and angular momentum over large distances through empty space. 
Maxwell's predictions were magnificently verified in the experiments of Hertz, 
confirming the reality and characteristics of electromagnetic waves \ct{HH}. 
From these results it became clear, for example, that light is just a special 
variety of such waves. Therefore optical and electromagnetic phenomena have a
common origin and can be described in a single theoretical framework. 

The concept of field has found other applications in physics, for example in 
the phenomenological description of fluids and gases. Treating them as 
continua, one can describe the local pressure and temperature as fields, with 
local variations in these quantities propagating through the medium as sound 
waves or heat waves. 

As in electrodynamics, also in gravity the concept of field has taken a 
central place. What Maxwell achieved for electromagnetism, was 
accomplished by Einstein in the case of gravity \ct{AE}: to obtain a complete 
description of the forces in terms of space- and time-dependent 
fields. This field theory is known as the general theory of relativity. 
One of the most remarkable aspects of this theory is, that it provides an 
interpretation of gravitational phenomena in terms of the geometry of 
space-time. Many detailed presentations of the geometrical description of
space-time can be found in the literature, including a number of books
included in the references at the end of these lecture notes 
\ct{AE2}-\ct{Wald}. A general outline of the structure of the theory 
is presented in the following sections.


\section{Geometrical interpretation of gravity}{\label{S1.3}} 

The first step in describing a local field, both in electrodynamics and 
gravity, is to specify the potentials. The force on a test particle at a 
certain location is then computed from the gradients of these potentials.
In the case of gravity these quantities have not only a dynamical
interpretation, but also a geometrical one. Whereas the electromagnetic 
field is described in terms of one scalar and one vector potential, 
together forming the components of a four vector\footnote{We use greek 
letters $\mu,\nu,...$, taking values (0,1,2,3), to denote the space-time 
components of four vectors and tensors.} $A_{\mu}(x)$, the gravitational 
field is described by 10 potentials, which can be assembled in a symmetric 
four tensor $g_{\mu\nu}(x)$. This tensor has a geometrical interpretation
as the metric of space-time, determining invariant space-time intervals 
$ds$ in terms of local coordinates $x^{\mu}$:

\be
ds^2\, =\, g_{\mu\nu}(x)\, dx^{\mu} dx^{\nu}.
\label{1.4}
\ee

\nit
In the absence of gravity, space-time obeys the rules of Minkowski geometry
well-known from special relativity. In cartesian coordinates $(ct,x,y,z)$ the 
metric of Minkowski space is 

\be
\eta_{\mu\nu}\, =\, \mbox{diag}(-1,+1,+1,+1). 
\label{1.4.0}
\ee

\nit
Then the invariant $ds^2$ takes the form

\be
ds^2\, =\, \eta_{\mu\nu}\, dx^{\mu} dx^{\nu}\, 
       =\, - c^2 dt^2 + dx^2 + dy^2 + dz^2.
\label{1.4.1}
\ee

For a test particle, there is a simple physical interpretation of invariant 
space-time intervals measured along its world line, in terms of proper time 
measured by a clock in the local rest frame of the particle. As world lines 
are time-like, any interval along a world line satisifies $ds^2 < 0$, and the 
proper time interval $d\tau$ measured by a clock at rest with respect to the 
particle is given by


\be
c^2 d\tau^2\, =\, - ds^2.
\label{1.5.1}
\ee

\nit
The local matrix inverse of the metric is denoted by $g^{\mu\nu}(x)$:

\be
g^{\mu\nu}(x)\, g_{\nu\lb}(x)\, =\, \del^{\mu}_{\lb},
\label{1.5}
\ee

\nit
where $\del^{\mu}_{\lb}$ is the Kronecker delta, and the Einstein summation 
convention has been used. This convention implies that one should automatically
perform a full summation over any repeated upper and lower indices, like $\nu$ 
on the left-hand side of this equation. 

From the gradients of the potentials, i.e.\ of the metric tensor, one 
constructs a quantity known as the connection, with components 
$\Gam_{\mu\nu}^{\:\:\:\:\:\lb}$ given by the expression:

\be
\Gam_{\mu\nu}^{\:\:\:\:\:\lb}\, =\, \frac{1}{2}\, g^{\lb\kg}\, \lh
   \pl_{\mu} g_{\kg\nu} + \pl_{\nu} g_{\mu\kg} - \pl_{\kg} g_{\mu\nu} \rh.
\label{1.5.2}
\ee

\nit
At this point this expression may simply be considered a definition. It is
a useful definition because this combination of gradients of the metric 
occurs very often in equations in general relativity. The deeper mathematical
reason for this stems from the transformation properties of expressions for
physical quantities under local coordinate transformations. However, it is 
not necessary to discuss these aspects at this point. 

A physical argument for the importance of the connection is, that it gives
directly the gravitational acceleration of a test particle in a given 
coordinate system by the following prescription, due to Einstein: the world 
lines of point-like test particles in general relativity are time-like 
geodesics of space-time, the latter being considered as a continuous 
pseudo-euclidean space\footnote{ The term pseudo-euclidean here refers to 
the fact that the metric is not positive-definite, as it would be in a true 
euclidean space; space-time has a lorentzian signature $(-,+,+,+)$, which 
implies that a general metric $g_{\mu\nu}$ has one negative (time-like) and 
three positive (space-like) eigenvalues.} with metric $g_{\mu\nu}$. 
Time-like geodesics are lines along which the total proper time between two 
fixed events $\int d\tau$ is an extremum; such world lines are solutions of 
the equation of motion 

\be
\frac{d^2 x^{\mu}}{d\tau^2}\, +\, \Gam_{\lb\nu}^{\:\:\:\:\:\mu}\, 
\frac{d x^{\nu}}{d\tau} \frac{d x^{\lb}}{d\tau}\, =\, 0.
\label{1.6}
\ee

\nit
A geometrical interpretation of the connection is therefore that it defines 
geodesics. As concerns its dynamical interpretation, there is some similarity
of eq.(\ref{1.6}) with the Lorentz force in electrodynamics in that the proper
acceleration depends on the four velocity $\dot{x}^{\mu}$ (we use an overdot 
to denote a derivative w.r.t.\ proper time). However, whereas the Lorentz 
force is linear in the four velocity, the gravitational acceleration depends 
quadratically on the four velocity. The coefficients of this quadratic
term are given by the connection, which therefore directly determines the 
force. Notice, that the gravitational acceleration does not involve the mass
of the test particle. This is the mathematical content of the famous {\em 
equivalence principle}, which states that in a fixed gravitational field all 
bodies fall with the same acceleration, independent of their mass. 

Eqs.(\ref{1.6}) and (\ref{1.5.2}) express the force on a test particle in
terms of a field (the connection), and the field in terms of potentials
(the metric). This provides the basis for the field theory of gravity
formulated by Einstein in his theory of general relativity. 

What is still lacking here of course is a set of equations determining the 
fields or potentials in terms of given sources, like Maxwell's equations 
allow one to compute the electromagnetic fields in terms of charges and 
currents. General relativity provides such equations; they are known as the 
Einstein equations, and they determine the gravitational fields arising from 
given distributions of mass-energy and momentum. These distributions, the 
sources of the gravitational fields, are described by a symmetric tensor 
$T_{\mu\nu}(x)$ with 10 independent components, equal to the number of 
independent components of the metric; $T_{\mu\nu}$ is called the 
energy-momentum tensor. In order to give a concise formulation of Einstein's
equations, it is useful to first introduce one more geometrical concept, that 
of curvature.

\section{Curvature}

Curvature is a important concept, because it characterizes the space-time 
geometry in a way which is basically coordinate independent. In order to 
illustrate the idea, we first present a heuristic discussion. Then we turn 
to mathematical definitions, which allow us to write Einsteins equations in 
a compact way with a direct and elegant geometrical interpretation. 

Curvature is defined in terms of the properties of surfaces; it is a 
measure of their deviation from a flat plane. Curvature can be expressed 
conveniently in terms of the change of a vector when transported parallel 
to itself around a loop enclosing a two-dimensional surface element. 
In a plane, displacement of a vector parallel to itself will always 
result in the same vector when you return to the starting point: 
there is absolute parallelism, but no curvature. In a curved surface 
this is no longer true. Consider the example of a sphere, a surface 
of constant curvature. If a vector is moved southward from the north 
pole parallel to itself, along a great circle, it ends up on the 
equator cutting it at a right angle. Now transport it along the equator 
over an arc of angular extension $\th$, always keeping at a right angle. 
Finally, move it back to the north pole along a great circle, keeping 
it parallel to the great circle and to itself. It then ends up at the 
north pole rotated by an angle $\th$ with respect to its original 
orientation. Thus parallel transport of a vector along a closed loop 
on a curved surface does not leave the vector invariant in general. 

In the example of the sphere, the rotation of the vector is proportional to 
the distance traveled along the equator, as measured by the angle $\th$. This 
is also proportional to the area enclosed by the loop consisting of the two 
sections of great circles through the north pole and the arc of the equator.
For a sphere with radius $R$, the change $dV$ in a vector $V$ when the loop 
encloses an area $dA = R^2 d\th$ is 

\be
dV = V d\th = \frac{V}{R^2}\, dA \equiv K V dA.
\label{1.7}
\ee

\nit
The constant of proportionality $K = 1/R^2$  between the relative change in
the vector $dV/V$ and the change in the area $dA$ is a measure of the intrinsic 
curvature of the surface, known as the Gaussian curvature. Note, that the 
Gaussian curvature is large when the radius of the sphere is small, and that it
vanishes in the limit $R \rightarrow \infty$, as one would expect intuitively. 
\vspace{2ex}

\nit
This idea can now be generalized to situations in higher-dimensional spaces. 
Of course, in a space of three or more dimensions, there are many surfaces
one can draw through a given point. Each of these surfaces may have its 
own curvature. Our first conclusion is therefore, that in general the 
curvature has many components. 

Fortunately, it is only necessary to consider curvature components in surfaces 
which are linearly independent. To this end, let us choose a locally 
non-degenerate coordinate system $x^{\mu}$ and consider in particular the 
surfaces defined by keeping all coordinates constant except two, say 
$x^{\mu}$ and $x^{\nu}$.

Let $d \Sg^{\mu\nu} = - d \Sg^{\nu\mu}$ be the area of an oriented surface 
element in the $x^{\mu}$-$x^{\nu}$-plane which contains the point with 
coordinates $(x_0)$. Any vector with components $V^{\lb}$ transported parallel
to itself around the loop defined by the circumference of this surface element 
now changes to first order by an amount

\be
d V^{\lb} = - \frac{1}{2}\, R_{\mu\nu\kg}^{\:\:\:\:\:\:\:\:\lb}(x_0)\, 
               V^{\kg} d \Sg^{\mu\nu}.
\label{1.8}
\ee

\nit
The constants of proportionality $R_{\mu\nu\kg}^{\:\:\:\:\:\:\:\:\lb}(x_0)$ 
define a tensor known as the Riemann curvature tensor at the location $(x_0)$. 
A comparison with eq.(\ref{1.7}) shows, that the Riemann tensor is a 
higher-dimensional generalization of the Gaussian curvature. From eq.(\ref{1.8}) 
it follows immediately, that a space-time is completely flat if and only if all 
components of the Riemann curvature tensor vanish. 

Defining parallel transport of a vector along a line element $dx^{\lb}$ in 
terms of the Riemann-Christoffel connection (\ref{1.5.2}):

\be
d V^{\mu}\, =\, - d x^{\lb}\, \Gm{\lb}{\nu}{\mu}\, V^{\nu},
\label{1.8.1}
\ee 

\nit
a direct computation for an infinitesimal closed loop gives the result that the 
components of the Riemann tensor can be expressed as 

\be
R_{\mu\nu\kg}^{\:\:\:\:\:\:\:\:\lb}\, =\, \pl_{\mu} 
   \Gam_{\nu\kg}^{\:\:\:\:\:\lb}\, -\, \pl_{\nu} \Gam_{\mu\kg}^{\:\:\:\:\:\lb}\,
   -\, \left[ \Gam_{\mu}, \Gam_{\nu} \right]_{\kg}^{\:\:\lb},
\label{1.9}
\ee

\nit
where the square brackets denote an ordinary matrix commutator of two 
connection components, considered as $4 \times 4$ matrices 
$(\Gam_{\ag})_{\kg}^{\:\:\lb}$, the first one with $\ag = \mu$, the second one 
with $\ag = \nu$.

Using eq.(\ref{1.5.2}) for the connection, we can ultimately express the 
curvature in terms of the metric and its first and second derivatives.
It may then be checked from this explicit expression that it identically 
satisfies the relation

\be
R_{\mu\nu\lb}^{\:\:\:\:\:\:\:\:\kg}\, +\, R_{\nu\lb\mu}^{\:\:\:\:\:\:\:\:\kg}\,
  +\, R_{\lb\mu\nu}^{\:\:\:\:\:\:\:\:\kg}\, =\, 0.
\label{1.9.1}
\ee

\nit
This relation is known as the Bianchi identity. It is analogous to 
the homogeneous Maxwell-equation, which implies that the electric and magnetic 
fields can be obtained from a four-vector potential $A_{\mu}$. In a similar way 
the Bianchi identity for the curvature tensor implies that the curvature tensor 
can be obtained from a symmetric tensor $g_{\mu\nu}$.

We wish to emphasize here, that the curvature of space-time is {\em not} a 
measure for the strength of the gravitational fields or forces; rather, it 
is a measure for the {\em variation} of the gravitational fields in space and 
time, the gradients.

\section{The Einstein equations}{\label{S1.4}}

The Einstein equations are second order non-linear partial differential 
equations for the metric of space-time in terms of a given energy-momentum 
distribution. As a result, these equations describe variations of the 
fields in space and time, rather than the fields themselves. In view of
the role of curvature as a measure for such variations and the geometrical 
interpetation of gravitational forces, it is quite natural that the 
Einstein equations should admit an interpretation as equations for the 
curvature of space-time. However, rather than the full Riemann tensor, 
it turns out that these equations involve only its contracted forms, the 
Ricci tensor $R_{\mu\nu}$ and the curvature scalar $R$:

\be
R_{\mu\nu}\, =\, R_{\mu\lb\nu}^{\:\:\:\:\:\:\:\:\lb}, \hspace{3em}
R\, =\, R_{\mu}^{\:\:\mu}\, =\, g^{\mu\nu}\, R_{\mu\nu}. 
\label{1.10}
\ee

\nit
Note that we adhere to the general convention that contraction with an 
inverse metric can be used to raise an index of a vector or tensor, turning 
a covariant component into a contravariant one; similarly contraction of an 
upper index on a vector or tensor with the metric itself is used to lower it
to make a covariant component out of a contravariant one. 

The reason that only the contracted forms of the Riemann curvature appear 
in the Einstein equations is, that in four-dimensional space-time the 
Riemann curvature tensor has too many components, twice as many as the 
metric. Therefore fixing the metric components in terms of the full 
Riemann tensor would generally lead to an overdetermined system of equations. 
In contrast, the Ricci tensor is symmetric: $R_{\mu\nu} = R_{\nu\mu}$, and 
has 10 independent components, precisely equal to the number of metric 
components to be solved for. It is therefore to be expected that the Einstein 
equations take the form of an equation for the Ricci tensor. Indeed, 
Einstein's equations for the gravitational fields can be written in the simple 
form

\be
R_{\mu\nu}\, -\, \frac{1}{2}\, g_{\mu\nu}\, R\, =\,  
                                            -\frac{8 \pi G}{c^4}\, T_{\mu\nu},
\label{1.11}
\ee

\nit
or equivalently:

\be
R_{\mu\nu}\, =\, -\frac{8 \pi G}{c^4}\, \lh T_{\mu\nu} - 
                                               \frac{1}{2}\, g_{\mu\nu} T \rh,
\label{1.11.1}
\ee

\nit
where $T = T_{\mu}^{\:\:\mu} = g^{\mu\nu} T_{\mu\nu}$. Notice the appearance 
of Newton's constant on the right-hand side of the equations. Of course, in 
empty space-time $T_{\mu\nu} = 0$; the second version of Einstein's equations 
(\ref{1.11.1}) then implies that the  Ricci tensor vanishes:

\be
R_{\mu\nu}\, =\, 0.
\label{1.12}
\ee

\nit
Space-time geometries which satisfy these conditions are some-times called
{\em Ricci-flat}. The most interesting aspect of these equations is, that 
an empty space-time can still support non-trivial gravitational fields: the 
Riemann curvature tensor can have non-zero components even if its contracted 
form, the Ricci tensor, is zero everywhere. 

This observation is important, because it lies at the heart of the 
theoretical arguments for the existence of gravitational waves. Indeed, 
as we discuss in more detail later on, one can find non-trivial solutions 
of the Einstein equations representing lumps in the gravitational field 
which travel at the speed of light and transport a finite amount of 
energy and momentum per unit of volume from one flat part of empty space 
to another flat part of empty space. 
 
There is a modified version of Einstein's equations in which the 
gravitational field itself creates a non-vanishing energy-momentum tensor,
even in the absence of matter. This gravitational field behaves like a 
homogeneous continuum with constant density and pressure (one of them negative), 
satisfying the equations                               

\be
R_{\mu\nu}\, =\, \frac{8 \pi G}{c^4}\, g_{\mu\nu} \Lb,
\label{1.13}
\ee

\nit
with $\Lb$ a constant. Such an equation arises if the energy-momentum tensor is

\be
T_{\mu\nu}\, =\, g_{\mu\nu} \Lb .
\label{1.13.1}
\ee

\nit
The constant $\Lb$ is known as the {\em cosmological constant}. 
Contraction of eq.(\ref{1.13}) with the inverse metric gives 

\be
R\, =\, \frac{32 \pi G}{c^4}\, \Lb.
\label{1.14}
\ee

\nit
This shows that in the presence of a cosmological constant empty space-time 
has a constant non-zero scalar curvature. Depending on the sign of the 
cosmological constant, eq.(\ref{1.13}) then admits solutions of Einstein's 
equations corresponding to empty space-times in continuous expansion or 
contraction. This modified version of Einstein's equations is especially 
interesting with regard to cosmological applications. 

Of course in the general case there is a contribution to the 
energy-momentum tensor from all matter and energy which happens to be 
present in the part of the universe we wish to describe. The precise
form of the energy-momentum tensor depends on the kind of matter
or radiation which constitutes the source of the gravitational field. 
However, it is very often justified and convenient to treat matter
and radiation as an ideal fluid, the energy-momentum tensor of which
depends only on the mass- and pressure-density and its flow, as 
decribed by the local four velocity of an element of fluid at location
with coordinates $(x)$. Denoting the mass density by $\rho(x)$, the
pressure density by $p(x)$, and the local four velocity by $u^{\mu}(x)$,
the energy-momentum tensor then takes the form

\be
T_{\mu\nu}\, =\, p g_{\mu\nu}\, +\, \lh p + \rho \rh u_{\mu} u_{\nu}.
\label{1.15}
\ee

\nit
Comparison with eq.(\ref{1.13.1}) shows, that the cosmological constant
can be reobtained from an ideal fluid with $p = - \rho = \Lb$. 

\section{The action principle}{\label{S1.6}}

The Einstein equations (\ref{1.11}) can be obtained from a variational
principle; that is, they follow by requiring an action $S$ to be stationary 
under variations $\del g_{\mu\nu}$ of the metric: $\del S = 0$. The action
for the gravitational field equations, including a coupling to material 
energy-momentum, is

\be
S\, =\, -\frac{1}{2c}\, \int d^4 x\, \sqrt{ - g}\, \lh \frac{c^4}{8 \pi G}\, R 
        + g^{\mu\nu} \Th_{\mu\nu} \rh.
\label{1.16}
\ee

\nit
Here $\Th_{\mu\nu}(x)$ represents the specific source term, but generally it 
is not the energy-momentum tensor itself; rather, the energy-momentum tensor is 
given in terms of $\Th_{\mu\nu}$ and its covariant trace $\Th = 
\Th_{\mu}^{\:\:\mu}$ by

\be
T_{\mu\nu} = \Th_{\mu\nu} - \frac{1}{2}\, g_{\mu\nu} \Th.
\label{1.16.1}
\ee

\nit
However, we consider $\Th_{\mu\nu}$ to be the independent variable, hence by
fiat there is no contribution from this tensor under variations with respect to 
the metric. Moreover, in eq.(\ref{1.16}) $g(x) = \det g_{\mu\nu}(x)$, and the 
minus sign is necessary because of the lorentzian signature of the metric, which 
implies the product of its eigenvalues to be negative everywhere. The proof of 
the action principle can be stated in a few lines, but it requires some 
intermediate results which we discuss first. 

To begin with, in stead of considering variations of the metric $g_{\mu\nu}$, 
one can equivalently use the variations of the inverse metric $g^{\mu\nu}$.
Indeed, because $g_{\mu\lb} g^{\lb\nu} = \del_{\mu}^{\lb}$, it follows that

\be
\del g_{\mu\lb} g^{\lb\nu}\, +\, g_{\mu\lb} \del g^{\lb\nu}\, =\, 0,
\label{1.17}
\ee

\nit
or 

\be
\del g_{\mu\nu}\, =\, - g_{\mu\lb} \del g^{\lb\kg} g_{\kg\nu}.
\label{1.18}
\ee

\nit
Thus the variation of the metric can be expressed in terms of the variation
of the inverse metric and vice versa. 

Next, we need a rule for computing the variation of the determinant $g$. This 
is obtained from the formula

\be 
\log \det M = \Tr \log M,
\label{1.19}
\ee

\nit
which holds for symmetric matrices $M$, as can easily be checked by 
diagonalizing $M$ and using the rule that the logarithm of the product equals 
the sum of the logarithms of the eigenvalues. From this equation we then 
derive

\be
\frac{1}{-g}\, \del (-g)\, =\,  g^{\mu\nu} \del g_{\mu\nu}\, 
            =\, - \del g^{\mu\nu} g_{\mu\nu}.
\label{1.20}
\ee

\nit
Finally, we observe that the Ricci tensor $R_{\mu\nu}$ is an expression
involving only the connection $\Gam_{\mu\nu}^{\:\:\:\:\:\lb}$. Hence

\be 
\del R\, =\, \del g^{\mu\nu}\, R_{\mu\nu}\, +\, g^{\mu\nu} \del R_{\mu\nu},
\label{1.21}
\ee

\nit
with the variation $\del R_{\mu\nu}$ expressible purely terms of the variation
of the connection $\del \Gam_{\mu\nu}^{\:\:\:\:\:\lb}$. The total variation
of the action now becomes 

\be
\ba{ll}
\del S = & \dsp{ -\frac{1}{2c}\, \int d^4 x\, \sqrt{ - g}\,  \del g^{\mu\nu}
\left[ \lh \frac{c^4}{8 \pi G}  R_{\mu\nu} + \Th_{\mu\nu} \rh - \frac{1}{2}
 g_{\mu\nu} \lh \frac{c^4}{8 \pi G} R + \Th \rh \right] } \\
  & \\
  & \dsp{ - \frac{1}{2}\, \int d^4 x\, \sqrt{ - g}\, \frac{\del R}{\del \Gam_{\mu\nu}^{\:\:\:\:\:\lb}}\, \del \Gam_{\mu\nu}^{\:\:\:\:\:\lb}. } 
\label{1.22}
\ea
\ee

\nit
The last term is to be interpreted in the sense that we vary $R$ with respect 
to the metric only via its dependence on the connection. However, it turns
out that if we insert the expression (\ref{1.5.2}) for the connection, this
whole variation adds up to a total derivative. As the action principle
applies to variations which vanish on the boundary, this term does not 
contribute to $\del S$. If we then require the variation of the action to 
vanish, we indeed obtain the Einstein equations:

\be
\ba{rll}
 \dsp{ \frac{c^4}{8 \pi G} \lh R_{\mu\nu} - \frac{1}{2} g_{\mu\nu} R \rh\,  
 +\, \Th_{\mu\nu} }\, -\, \frac{1}{2}\, g_{\mu\nu} \Th &  = & \\ 
   \\
\dsp{ \frac{c^4}{8 \pi G} \lh R_{\mu\nu} - \frac{1}{2} g_{\mu\nu} R \rh\,
 +\, T_{\mu\nu} } & = & 0. \\
\label{1.23}
\ea
\ee

\nit
The equation with the cosmological constant is obtained by making the 
replacement $ g^{\mu\nu}\Th_{\mu\nu} = \Th \rightarrow 2 \Lb$ in the action.








 




==> dyn.tex <==
 \chapter{Dynamics of space-time \label{C3}}

\section{Classical solutions of the gravitational field equations 
         \label{S3.1}}

The Einstein equations (\ref{1.11}) describe the gravitational fields
generated by a specific distribution of material sources, as described
by the energy-momentum tensor $T_{\mu\nu}$. In two or three dimensions,
these fields carry at best a finite number of physical degrees of 
freedom, related to the sources and/or the topology \ct{Wit1}. In four 
or higher-dimensional space-time the gravitational field is a fully 
dynamical system with infinitely many degrees of freedom. In particular, 
dynamical gravitational fields can exist in the absence of material 
sources, in empty space-time. In the geometrical interpretation of 
general relativity such fields represent the intrinsic dynamics of 
space-time itself. 

In eq.(\ref{1.8}) the curvature tensor was defined in terms of the 
parallel transport of a vector around a closed curve. A manifold 
is called flat if after parallel transport around an arbitrary 
closed curve in the manifold the image of any vector coincides with 
the original. Therefore a necessary and sufficient condition for a 
manifold to be flat near a given point is that the components of the 
Riemann tensor $R_{\mu\nu\kg}^{\:\:\:\:\:\:\:\lb}$ vanish there. 
This condition is more general than to require that the metric takes 
the form

\be
ds^2\, =\, \pm dx_0^2\, +\, \sum_{i=1}^n\, dx_i^2,
\label{c3.1}
\ee

\nit
with the sign depending on the euclidean or lorentzian signature of the 
manifold. Indeed, in any differentiable manifold one can always find a local 
coordinate system in the neighborhood of a given point, in which the line 
element can be diagonalized to this form, but this is not generally the 
case globally. Even in cases in which it can be done globally, eq.(\ref{c3.1}) 
is not the most general solution of the Einstein equations for flat empty 
space-time, because it is still allowed to perform an arbitrary local change of 
co-ordinates in this metric. The flatness-criterion introduced above, 
amounting to the vanishing of the Riemann-curvature, is more useful as it 
holds in any co-ordinate system and in any topology. 

The existence of non-trivial solutions of the Einstein equations with 
vanishing cosmological constant in matter-free regions of space-time is 
possible because vanishing of the Ricci-tensor does not imply a vanishing 
of all components of the Riemann-tensor. A formal mathematical criterion 
for distinguishing solutions of the Einstein equations in empty space from 
those with material sources is through the Weyl curvature tensor, defined 
as the completely traceless part of the Riemann tensor:

\be
\ba{lll}
W_{\mu\nu\kg\lb} & = & \dsp{ R_{\mu\nu\kg\lb}\, -\, \frac{1}{(d-2)} 
  \lh g_{\mu\kg} R_{\nu\lb} - g_{\nu\kg} R_{\mu\lb} - g_{\mu\lb} R_{\nu\kg}
      + g_{\nu\lb} R_{\mu\kg} \rh\, }\\
 & & \\
 & & \dsp{ +\, \frac{1}{(d-1)(d-2)}\,
  \lh g_{\mu\kg} g_{\nu\lb} - g_{\mu\lb} g_{\nu\kg} \rh\, R. }
\ea
\label{c3.2}
\ee

\nit
Here $d$ is the dimensionality of the manifold. If we similarly define
$W_{\mu\nu}$ as the traceless part of the Ricci tensor:

\be
W_{\mu\nu} = R_{\mu\nu} - \frac{1}{d}\, g_{\mu\nu} R,
\hspace{3em} W_{\mu\nu} = W_{\nu\mu}, \hspace{3em} W_\mu^{\:\:\mu} = 0,
\label{c3.3}
\ee

\nit
then we obtain a complete decomposition of the Riemann tensor in terms of 
traceless components and the Riemann scalar:

\be 
\ba{lll}
R_{\mu\nu\kg\lb} & = & \dsp{ W_{\mu\nu\kg\lb}\, +\, \frac{1}{(d-2)}\, 
  \lh g_{\mu\kg}  W_{\nu\lb} - g_{\nu\kg} W_{\mu\lb} - g_{\mu\lb} W_{\nu\kg}
      + g_{\nu\lb} W_{\mu\kg} \rh\, }\\
 & & \\
 & & \dsp{ +\, \frac{1}{d(d-1)}\, \lh g_{\mu\kg} g_{\nu\lb} - 
           g_{\mu\lb} g_{\nu\kg} \rh\, R. }
\ea
\label{c3.4}
\ee

\nit
This decomposition allows a classification of the solutions of the 
Einstein equations according to which of the independent components 
$(W_{\mu\nu\kg\lb}, W_{\mu\nu}, R)$ vanish and which don't. In particular,  
metrics for which only the Weyl tensor is non-vanishing are solutions of 
the source-free Einstein equations $R_{\mu\nu} = 0$. On the other hand, 
there also exist manifolds for which the only non-zero component is the
Riemann scalar $R$, whilst the Weyl tensor and traceless Ricci tensor
vanish: the $n$-spheres $x_0^2 + x_1^2 + \dots + x_n^2 = \rg^2$, and all 
two-dimensional surfaces. For the $n$-spheres this follows essentially 
from the spherical symmetry, which implies the absence of any prefered 
direction, in combination with the permutation symmetries between the 
components of the Riemann curvature tensor. 

For two-dimensional manifolds, it is always possible to write the 
Riemann tensor as

\be 
R_{\mu\nu\kg\lb}\, =\, 
 \frac{1}{2}\, g\, \ve_{\mu\nu}\, \ve_{\kg\lb}\, R\, =\,
 \frac{1}{2}\, \lh g_{\mu\kg} g_{\nu\lb} - g_{\nu\kg} g_{\mu\lb} \rh\, R. 
\label{c3.4.1}
\ee

\nit
For the (torsion-free) riemannian and pseudo-riemannian manifolds we 
consider in higher dimensions $(d \geq 3)$, the number of independent 
components of the Riemann tensor $R_{\mu\nu\kg\lb}$, taking account of all 
its symmetries, is given by:

\be
N[ R_{\mu\nu\kg\lb} ]\, =\, \frac{d^2(d^2 - 1)}{12}.
\label{c3.5}
\ee

\nit
This is counted as follows: the Riemann tensor is anti-symmetric in each
of the index pairs $[\mu\nu]$ and $[\kg\lb]$. Hence $R_{[\mu\nu][\kg\lb]}$
may be considered as a square matrix of dimension $n = d(d-1)/1$. Also as
an $(n \times n)$-matrix it is symmetric under interchange of these index 
pairs. As such it has $n(n+1)/2$ independent elements. Finally the cyclic 
symmetry in the first three (lower) indices of the fully covariant 
components of the Riemann tensor expressed by the Bianchi identity 
(\ref{1.9.1}) adds $d(d-1)(d-2)(d-3)/4!$ algebraic constraints, eliminating
an equal number of independent components. Combining these results one finds 
precisely the number $N[ R_{\mu\nu\kg\lb} ]$ in eq.(\ref{c3.5}) above. 

For $d \geq 3$ the number of components of the traceless Ricci tensor and 
Riemann scalar is

\be
N[ W_{\mu\nu} ]\, =\, \frac{d(d+1)}{2}\, -\, 1. \hspace{3em}
 N[ R ]\, =\, 1.
\label{c3.6}
\ee

\nit
(for $d = 2$ the Riemann curvature tensor has only one independent 
component, corresponding to the Riemann scalar). Therefore for $d \geq 3$ 
the number of independent components of the Weyl tensor is 

\be
N[ W_{\mu\nu\kg\lb} ]\, =\, \frac{1}{12}\, d(d+1)(d+2)(d-3).
\label{c3.7}
\ee

\nit
Clearly this vanishes for $d = 3$, and is positive non-zero only for 
$d \geq 4$. Thus we find indeed that non-trivial dynamical solutions 
to the source-free Einstein equations can exist only in space-times of 
dimensions $d \geq 4$. As the minimal case $d = 4$ happens to be the 
number of dimensions of our (macroscopic) world, we observe that for this 
case the Weyl tensor and the Ricci tensor each have 10 algebraically 
independent components. Therefore half of the components of the curvature 
are determined by the material sources, whilst the other half describes 
the intrinsic dynamics of space-time. 

In the geometrical interpretation of the gravitational field and its
dynamics, Einstein's famous principle of the equivalence of accelerations 
and local gravitational fields can be formulated as the hypothesis that 
space-time is a manifold, in each point of which one can establish a 
locally flat (cartesian) coordinate system of the form (\ref{c3.1}). Of 
course a fully geometric interpretation of all of physics, and also the 
equivalence principle, breaks down in those points or regions where 
material sources are located\footnote{Attempts to explain matter as a 
manifestation of physics in higher-dimensional space-time, as in 
Kaluza-Klein models or the more sophisticated string theories, aim to 
redress this situation.}. But also solutions of the source-free Einstein
equations can violate the equivalence principle locally if there are 
singularities --- for example points where curvature invariants become 
infinite and/or the number of dimensions changes. Physics at these points 
is no longer described, at least not completely, by the Einstein 
equations, and space-time is not necessarily a manifold in the strict 
sense. In some cases it can still be a manifold with boundaries, where 
specific boundary conditions hold; but these boundary conditions then 
represent external data and the gravitational field is not determined by 
general relativity alone.  

Nevertheless singular solutions are important because they are relevant 
for physics as we observe it in the universe: cosmological solutions of 
the Friedmann-Robinson-Walker type with a `Big Bang'-singularity, and  
black-hole solutions describing stellar collapse. The singularities in 
these cases are not necessarily physical, as the short-distance physics
may be regulated by Planck-scale modifications of the theory, which are 
presently unobservable. However that may be, here we simply accept the 
possibility of singularities and discuss examples of both non-singular 
and singular geometries arising as solutions of the Einstein equations. 
They illustrate many interesting aspects of gravitational physics.  

\section{Plane fronted waves \label{S3.2}}

To show that in four dimensions non-trivial gravitational fields can 
indeed propagate through empty space-time, we now consider a class 
of solutions known in the literature as plane-fronted gravitational waves 
\ct{Bondi1,Ehlers1}. This name derives from the property that there is a 
co-ordinate system in which these field configurations $(i)$ move with the 
speed of light along a straight line; $(ii)$ have a flat planar wave front,
and $(iii)$ are of finite duration. When discussing the physical 
properties of these solutions it will become clear that these wave-like
solutions actually behave more like dynamical domain walls. 

We construct a planar wave solution with the direction of motion along the 
$x$-axis, and the transverse directions defined by the $(y,z)$-plane. Thus 
we look for solutions of the Einstein equations of the form 

\be
g_{\mu\nu}(\vec{x},t)\, =\, \lh \ba{cc}
                              \ba{cc}
                               -1 &   \\
                                  & 1 \\
                              \ea          & \mbox{\bf 0} \\
                              \mbox{\bf 0} & \ba{cc}
                                              f^2(x,t) &          \\
                                                       & g^2(x,t) \\
                                             \ea                     
                        \ea \rh.
\label{2.1}
\ee

\nit
The corresponding space-time line-element is

\be
ds^2\, =\, - c^2 dt^2\, +\, dx^2\, +\, f^2(x,t) dy^2\, +\, g^2(x,t) dz^2.
\label{2.2}
\ee

\nit
We observe the following properties of these metrics: \nl
-- in the $(x,t)$-plane space-time is flat (Minkowskian); \nl
-- in the $y$- and $z$-directions space-time is generally not flat, but the 
value of the metric depends only on the distance along the $x$-axis and on 
time, not on the values of $y$ or $z$ themselves. Hence in the co-ordinate 
system chosen the components of these gravitational potentials are the same 
everywhere in the $(y,z)$-plane. In particular they do not fall off to unity 
at spatial infinity, showing that the space-time is not asymptotically 
Minkowskian at large space-like distances. Of course, they share this 
property with plane electromagnetic waves, which at a fixed time also have 
the same amplitude everywhere in the transverse directions; \nl
-- the metric has no inverse if $f = 0$ or $g = 0$; then the connections 
are singular. We must take special care when this happens. 

With the {\em Ansatz} (\ref{2.1}) for the metric one can compute the 
components of the connection using eq.(\ref{1.5.2}). Using the notation 
$x^{\mu} = (ct,x,y,z)$ for $\mu = (0,1,2,3)$, the non-vanishing components 
have been assembled in the following list:
\vspace{2ex}

\be
\fbox{ $ \ba{ll}
\dsp{ \Gm{0}{2}{2} = \Gm{2}{0}{2} = \frac{f_t}{cf},} & 
 \dsp{ \Gm{2}{2}{0} = \frac{1}{c}\, ff_t, } \\
        & \\
\dsp{ \Gm{0}{3}{3} = \Gm{3}{0}{3} = \frac{g_t}{cg},} & 
 \dsp{ \Gm{3}{3}{0} = \frac{1}{c}\, gg_t, } \\
        & \\
\dsp{ \Gm{1}{2}{2} = \Gm{2}{1}{2} = \frac{f_x}{f},} & \Gm{2}{2}{1} = - ff_x,\\
        & \\
\dsp{ \Gm{1}{3}{3} = \Gm{3}{1}{3} = \frac{g_x}{g},} & \Gm{3}{3}{1} = - gg_x.\\ 
       \ea $ }
\label{2.3} 
\ee  

\nit
The next step in solving the Einstein equations is to compute the components
of the Riemann curvature tensor using eq.(\ref{1.9}). The only independent 
covariant components $R_{\mu\nu\lb\kg} = R_{\mu\nu\lb}^{\:\:\:\:\:\:\:\:\rho} 
g_{\rho\kg}$ not identically zero are the following ones:

\be
\fbox{ $ \ba{ll}
\dsp{ R_{0202} = \frac{1}{c^2}\, ff_{tt},} & 
         \dsp{ R_{0303} = \frac{1}{c^2}\, gg_{tt}, } \\
        & \\
R_{1212} = ff_{xx}, & R_{1313} = gg_{xx}, \\
        & \\
\dsp{ R_{0212} = \frac{1}{c}\, ff_{tx},} &
         \dsp{ R_{0313} = \frac{1}{c}\, gg_{tx}, } \\
        & \\
\dsp{ R_{2323} =  fg ( f_x g_x - \frac{1}{c^2}\, f_t g_t). } & \\
      \ea $}
\label{2.4} 
\ee

\nit
Before discussing the general solution of the Einstein equations for this 
class of metrics, we first use the above results to answer the question which 
of the metrics singled out by the {\em Ansatz} (\ref{2.1}) describe flat 
Minkowski space. If we require all components of the curvature tensor 
(\ref{2.4}) to vanish independently, the most general solution for $f(x,t)$ 
and $g(x,t)$ is

\be
\ba{lll}
f(x,t) & = & a\, +\, p x\, +\, r ct,  \\
g(x,t) & = & b\, +\, q x\, +\, l ct,
\ea
\label{2.4.1}
\ee

\nit
with the additional constraint

\be
pq = rl. 
\label{2.4.2}
\ee

\nit
Thus metrics of the form (\ref{2.1}), and corresponding line-elements 
(\ref{2.2}), describe a flat space-time if $f$ and $g$ are linear functions 
of $x$ and $t$, with the additional constraint (\ref{2.4.2}) between their
co-efficients. 
\vspace{2ex}

\nit
The components of the Ricci tensor $R_{\mu\nu}$ now follow by taking a 
covariant trace as in eqs.(\ref{1.10}). The non-vanishing ones are
\vspace{2ex}

\be
\fbox{ $ \ba{l}
  \dsp{ R_{00}\, =\, \frac{1}{c^2}\, \lh \frac{f_{tt}}{f}\, +\, 
                     \frac{g_{tt}}{g} \rh, }\\
        \\
  \dsp{ R_{01}\, =\, R_{10}\, =\, \frac{1}{c}\, \lh \frac{f_{tx}}{f}\, +\,
                                  \frac{g_{tx}}{g} \rh, }\\
        \\
  \dsp{ R_{11}\, =\, \frac{f_{xx}}{f}\, +\, \frac{g_{xx}}{g}, }\\
        \\
  \dsp{ R_{22}\, =\, f \lh f_{xx} - \frac{1}{c^2}\, f_{tt} \rh\, +\, 
                 \frac{f}{g}\, \lh f_x g_x - \frac{1}{c^2} f_t g_t  \rh, }\\
        \\
  \dsp{ R_{33}\, =\, g \lh g_{xx} - \frac{1}{c^2}\, g_{tt} \rh\, +\, 
                  \frac{g}{f}\, \lh f_x g_x - \frac{1}{c^2}\, f_t g_t \rh, }
      \ea $}
\label{2.5}
\ee
\vspace{2ex}

\nit
In the absence of material sources Einstein's equations require the Ricci 
tensor to vanish. Assuming $f$ and $g$ themselves not to vanish identically, 
some manipulation of these equations then leads to the following five 
necessary and sufficient conditions:

\be
\ba{lll}
\dsp{ f_{xx} - \frac{1}{c^2}\, f_{tt} } & = & 0, \\
  & & \\
\dsp{ g_{xx} - \frac{1}{c^2}\, g_{tt} } & = & 0, \\
  & & \\
\dsp{ f_x g_x - \frac{1}{c^2}\, f_t g_t } & = & 0, \\
  & & \\
g f_{xx} + f g_{xx} & = & 0, \\
  & & \\
g f_{tx} + f g_{tx} & = & 0.
\ea
\label{2.6}
\ee

\nit
The first two equations are free wave equations in two-dimensional $(x,t)$ 
space. They imply that $f$ and $g$ can be decomposed into left- and 
right-moving waves:

\be
\ba{lll}
f(x,t) & = & f_{+}(x + ct)\, +\, f_{-}(x - ct), \\
  &  &  \\
g(x,t) & = & g_{+}(x + ct)\, +\, g_{-}(x - ct),
\ea
\label{2.7}
\ee

\nit
where $(f_{-}(\xi), g_-(\xi))$ and $(f_+(\eta), g_+(\eta)$ are functions 
only of the single lightcone variable $\xi = x - ct$, and $\eta = x + ct$, 
respectively. Each of these components then satisfies the wave equation by 
itself, and at this stage they can be taken to be completely independent. 
The only ambiguity here is that a possible constant term can be divided in 
an arbitrary way between the left- and right-moving components of the 
solution. 
 
If we now substitute this decomposition of $f$ and $g$ in the third equation
(\ref{2.6}), and assume that the first derivatives of the components with 
respect to $u$ or $v$ (i.e.\ $f_{\pm}^{\prime}$ and $g_{\pm}^{\prime}$) are 
all non-zero, then the only solutions of the Einstein equations correspond to 
flat Minkowski space. This can be seen by dividing the equation by 
$\pr{g}_{+} \pr{g}_{-}$ to obtain

\be
\frac{f_{+}^{\prime}}{g_{+}^{\prime}}\, =\, - 
                        \frac{f_{-}^{\prime}}{g_{-}^{\prime}}\, =\, \lb,
\label{2.8}
\ee

\nit
where $\lb$ on the right-hand side of the last equality is a finite, non-zero
constant. This last equality holds because the two previous expressions are 
functions of different variables, hence they can be identically equal only if 
they are constant. It then follows, that

\be
f_{+}^{\,\prime}\, =\, \lb g_{+}^{\,\prime}, \hspace{3em}
f_{-}^{\,\prime}\, =\, - \lb g_{-}^{\,\prime}.
\label{2.9}
\ee

\nit
Inserting these results into the last two equations (\ref{2.6}), addition
and subtraction gives the equivalent conditions

\be
\lh \lb g + f \rh\, g_{+}^{\,\prime\prime}\, =\, 0, \hspace{3em}
\lh \lb g - f \rh\, g_{-}^{\,\prime\prime}\, =\, 0.
\label{2.10}
\ee

\nit
The solution $g_{+}^{\,\prime\prime} = g_{-}^{\,\prime\prime} =  0$ implies
$f_{+}^{\,\prime\prime} = f_{-}^{\,\prime\prime} =  0$. This leads to linear 
dependence of $f$ and $g$ on $x$ and $t$: they are of the form (\ref{2.4.1}), 
(\ref{2.4.2}) and correspond to flat Minkowski space. 

On the other hand, in case one of the second derivatives 
$g_{\pm}^{\,\prime\prime}$ is non-zero, one of the co-efficients $(\lb g 
\pm f)$ must vanish; note that they cannot vanish simultaneously for 
non-zero $f$ and $g$. Hence eq.(\ref{2.10}) gives either 

\be
f\, =\, \lb g\, \hspace{3em} \mbox{and} \hspace{3em}
g_{+}^{\,\prime\prime}\, =\, f_{+}^{\,\prime\prime}\, =\, 0, 
\label{2.11}
\ee

\nit
or

\be
f\, =\, - \lb g\, \hspace{3em} \mbox{and} \hspace{3em}
g_{-}^{\,\prime\prime}\, =\, f_{-}^{\,\prime\prime}\, =\, 0. 
\label{2.12}
\ee

\nit
But combining this with the results (\ref{2.9}), we find again that all 
second derivatives must vanish and that the geometry is that of flat 
space-time.  

We conclude that in order to get non-trivial solutions, at least one of the 
first derivatives $\pr{f_{\pm}}$ or $\pr{g_{\pm}}$ must vanish. The last 
three equations (\ref{2.6}) then imply that, after absorbing any constants 
terms in the remaining components, the only solutions are

\be
f(x,t)\, =\,  f_{+}(x + ct), \hspace{3em} g(x,t)\, =\,  g_{+}(x + ct), \\
\label{2.13}
\ee

\nit
or 

\be
f(x,t)\, =\,  f_{-}(x - ct), \hspace{3em} g(x,t)\, =\,  g_{-}(x - ct), \\
\label{2.14}
\ee

\nit
with the additional condition

\be
\frac{f^{\prime\prime}}{f}\, +\, \frac{g^{\prime\prime}}{g}\, =\, 0.
\label{2.15}
\ee

\nit
Although $f$ and $g$ represent waves traveling either to the right or 
to the left at the velocity of light, the non-linear character of the
Einstein equations exemplified by the additional condition (\ref{2.15}) 
do not allow us to make arbitrary superpositions of these solutions. 
Interestingly, viewed as a two-dimensional theory in $(x,t)$-space $f$ and 
$g$ represent chiral bosons. Wherever necessary in the following we chose 
to work with right-moving fields $f(x,t) = f_{-}(\xi)$ and $g(x,t) = 
g_{-}(\xi)$ for definiteness. 

An example of a simple solution of eq.(\ref{2.15}) is \ct{Rindler}:

\be
\ba{lll}
f(x,t) & = & \cos k(x - ct)\, =\, \cos k\xi, \\
g(x,t) & = & \cosh k(x - ct)\, =\, \cosh k\xi.
\ea
\label{2.16}
\ee

\nit
Note that at $\xi = (2n + 1)\pi/2k$ the component $f$ has a zero, whilst 
the solution for $g(x,t)$ grows indefinitely with time or distance. However, 
this does neither imply that the geometry is singular, nor that the 
gravitational fields become arbitrarily strong: the apparent problems turn 
out to be coordinate artifacts. This point is discussed in detail in the next 
section. 

Let us consider a wave which reaches $x = 0$ at time $t = 0$, and extends
to $x = - L$, i.e.\ the solution (\ref{2.16}) holds for $-L \leq \xi  
\leq 0$. If $|kL| < \pi/2$ the metric components $f^2$ and $g^2$ are 
strictly positive. For $ \xi \geq 0$ space-time is flat; we can choose 
a co-ordinate system in which $f = g = 1$. Note that the wave solution 
(\ref{2.16}) assumes these same values at $\xi = 0$, whilst the first 
derivatives match as well. As a result the solutions are smoothly 
connected and satisfy the Einstein equations even at the boundary 
$\xi = 0$. 

For $\xi \leq -L$ space-time is again flat, but now we have to use the 
general solution (\ref{2.4.1}):

\be
\ba{cc}
       \ba{lll}
       f(x,t) & = & a\, +\, p(x - ct), \\
       g(x,t) & = & b\, +\, q(x - ct), 
       \ea &
              (x - ct) \leq -L.
\ea
\label{2.17}
\ee

\nit
The co-efficients $(a,b;p,q)$ in this domain of $(x,t)$ values are to be 
determined again by requiring the metric to be continuous and differentiable 
at the boundary $\xi = -L$ between the different domains of the solution. 
This condition is sufficient to guarantee that the Einstein equations are 
well-defined and satisfied everywhere. Imposing these requirements we find 

\be
\ba{ll} {\ba{rll}
         \cos kL & = & a\, -\, pL, \\
         & \\
         \cosh kL & = & b\, - qL, 
         \ea}                           &  {\ba{rll} 
                                            k \sin kL & = & p \\
                                            & \\
                                            - k \sinh kL & = & q.
                                            \ea} 
\ea
\label{2.18}
\ee

\nit
For $f$ and $g$ in the domain $(x - ct) \leq -L$ we obtain the result

\be
\ba{lll}
f(x,t) & = & \cos kL\, +\, k \lh L + x - ct \rh\, \sin kL , \\
  & & \\
g(x,t) & = & \cosh kL\, -\, k \lh L + x - ct \rh\, \sinh kL .
\ea
\label{2.19}
\ee

\nit
{\em Conclusion:} we have constructed a solution of the Einstein
equations in empty space which interpolates between two Minkowski
half-spaces, connected by a finite region of non-zero curvature, where 
the gravitational fields have non-zero gradients and test particles are 
accelerated with respect to the initial inertial frame. After passage
of the wave the test particles have acquired a finite, but constant 
velocity. This shows that they have been accelerated, but the acceleration 
has ceased after $t > (x + L)/c$. 
\vs

\nit
The plane-fronted wave constructed here is a well-defined solution of the 
equation $R_{\mu\nu} = 0$ everywhere, including the wave fronts $x = ct$ 
and $x = ct - L$, as the contributions of the metric components $g_{yy} = 
f^2$ and $g_{zz} = g^2$ always compensate each other in eq.(\ref{2.15}). 
However the Riemann curvature itself, which coincides with the Weyl 
curvature in this case, does not vanish everywhere. Indeed, we find from 
eq.(\ref{2.4}) 

\be
\ba{l}
R_{0202} = R_{1212} = \pm  R_{0212} = f f^{\prime\prime}, \\
 \\
R_{0303} = R_{1313} = \pm  R_{0313} = g g^{\prime\prime}, \\      
 \\
R_{2323} = 0. 
\ea 
\label{2.19.1} 
\ee

\nit
Inserting the explicit solution for $f$ and $g$ for each of the three 
regions $x > ct$, $- L < x - ct < 0$ and $x < ct - L$ one finds that the 
curvature is zero in the two Minkowski half-spaces before and after the 
wave, as expected, but finite and non-zero in the interior of the wave. 
Indeed, the second derivatives $f^{\prime\prime}$ and $g^{\prime\prime}$ 
have a finite discontinuity on the wave front of magnitude $\mp k^2$ at 
$x = ct$, and $-k^2 \cos kL$, resp.\ $k^2 \cosh kL$, at $x = ct - L$. This 
finite discontinuity then also appears in the curvature components, where 
it must be attributed to a finite discontinuity in the Weyl curvature, and
thus can not be attributed to a (singular) distribution of sources. But  
the Riemann-Christoffel connections, which depend only on the first 
derivatives of the metric, are continuous. Then the geodesics and the 
motions of test particles in the space-time described by the wave 
are continuous, and it follows that the jump in the Weyl curvature 
presents no physical inconsistencies. 

\section{Nature of the space-time \label{S3.3}}

The planar wave constructed above can be characterised as a region 
of non-vanishing curvature sandwiched between two flat space-times 
and propagating with the speed of light ---either in the positive 
or the negative $x$-direction--- such that one of the two flat 
space-time regions grows at the expense of the other. In this 
section we establish the relation between the two flat space-times, 
before and after the wave. The analysis shows that, although they 
are of course related by a general co-ordinate transformation, 
they are not related by a simple Lorentz transformation: a set of 
equidistant test particles carrying synchronised ideal clocks and 
thus defining an inertial co-ordinate system before the wave are 
neither equidistant nor synchronised in {\em any} inertial 
co-ordinate system after the wave. In this sense the two Minkowski 
space-times on either side of the region of non-zero curvature are 
inequivalent: in each the stability group of the vacuum, ---the 
Lorentz group of rigid transformations leaving the in-product of 
four-vectors invariant in each of the flat regions--- is embedded 
differently in the group of local co-ordinate transformations which 
constitutes the symmetry of the full theory.  

This situation is also encountered in scalar field theories with 
broken symmetry, when there is a boundary separating two domains 
with different vacuum expectation values of the field. One can 
even show that in some models these two forms of spontaneous 
symmetry breaking ---of a scalar field and of the gravitational 
field--- are connected \ct{jw1}. Therefore we find a new 
interpretation for the planar gravitational waves: they act as 
domain boundaries separating different, inequivalent flat-space 
solutions (`vacua') of the Einstein equations. These domain 
boundaries are dynamical: they are not static but move at the 
speed of light; it is shown below that these particular solutions 
are block waves of constant curvature. 

Regions of space-time enclosed by such dynamical boundaries clearly 
grow or shrink at the speed of light. If we consider our planar 
wave solution as an approximation to a more general domain-wall 
geometry with a radius of curvature large compared to the 
characteristic scale of the region of space-time we are interested 
in, then we can use it to describe the dynamics of gravitational 
domain structure, which has interesting implications for the physics 
of the early universe. 
 
Having sketched this general picture, I now turn to describe the 
sandwich structure of the planar wave geometry more precisely. A 
convenient procedure is to introduce new co-ordinates $X^{\mu} = (
cT,X,Y,Z)$ related to the original $x^{\mu} = (ct,x,y,z)$ by 

\be
\ba{lll}
c\,T & = & \dsp{ ct\, +\, \frac{\Lb}{2}, }\\
  & & \\
X & = & \dsp{ x\, +\, \frac{\Lb}{2}, }\\
  & & \\
Y & = & f y, \\
  & & \\
Z & = & g z, \\
\ea
\label{2.20}
\ee

\nit
where in terms of the original coordinates $x^{\mu}$  

\be
\Lb(x^{\mu})\, =\, y^2 f \pr{f}\, +\, z^2g \pr{g}.
\label{2.21}
\ee

\nit
This coordinate transformation takes an even simpler form when expressed 
in the (normalized) light-cone variables $(U,V)$:

\be 
\ba{llll}
U & = & \lh cT - X  \rh / \sqrt{2}& =\, \lh ct - x \rh/\sqrt{2} \, =\, u, \\
  & & & \\ 
V & = & \lh cT + X  \rh/\sqrt{2} & =\, \lh ct  + x + \Lb\rh/\sqrt{2} \,
    =\, v + \Lb/\sqrt{2}. 
\ea 
\label{2.21.1} 
\ee

\nit
Indeed the line-element (\ref{2.2}) now becomes

\be
\ba{lll}
ds^2 & = & - c^2 dt^2\, +\, dx^2\, +\, f^2 dy^2\, +\, g^2 dz^2 \\
  & & \\
  & = & - 2 dU dV - 2 K(U,Y,Z) dU^2 + dY^2 + dZ^2,
\ea
\label{2.22}
\ee

\nit
with 

\be
K(U,Y,Z) = -\, \frac{f^{\prime\prime}}{f}\, Y^2\, -\, 
         \frac{g^{\prime\prime}}{g}\, Z^2\, =\, \frac{g^{\prime\prime}}{g}\,
         \lh Y^2 - Z^2 \rh.
\label{2.22.1}
\ee

\nit
Both for $t < x/c$ and $t > (x + L)/c$ we have $f^{\prime\prime} = 
g^{\prime\prime} = 0$, and therefore the line element (\ref{2.22}) is 
manifestly flat Minkowskian on both sides of the planar wave. However, 
inside our particular wave solution one has

\be
\frac{f^{\prime\prime}}{f}\, =\, -\, \frac{g^{\prime\prime}}{g}\, 
  =\, -\, k^2.
\label{2.22.2}
\ee

\nit
Then $K = k^2 (Y^2 - Z^2)$, independent of $U$. The coordinate system
$X^{\mu}$ with the line-element (\ref{2.22}) is the closest one to an
inertial frame at all times for an observer at rest in the origin one can 
construct. Indeed, the point $x = y = z = 0$ corresponds to $X = Y = Z = 0$ 
at all times, and both before and after the wave the $X^{\mu}$ define a 
global inertial frame. Furthermore, inside the wave the new coordinate 
system deviates from an inertial frame only for large values of 
$(Y^2 - Z^2)$. We also observe that in this coordinate system the line 
element (\ref{2.22}) never becomes singular, showing the previous zero's 
of $\det g$, corresponding to zero's of $f(u)$, to be coordinate artifacts 
indeed.

Computing the various geometrical quantities: metric, connections and 
curvature components, in the new coordinates produces the following summary 
of results: \nl
-- The only non-vanishing components of the inverse metric are:

\be
\ba{ll}
g^{UV} = g^{VU} = - 1, &  g^{VV} = 2 K = 2 k^2(Y^2 - Z^2), \\
 & \\ 
g^{YY} = g^{ZZ} =  1. & 
\ea
\label{2.22.3}
\ee

\nit
-- The only non-vanishing components of the connection are:

\be
\ba{l}
\Gm{U}{U}{Y} = \Gm{Y}{U}{V} = \Gm{U}{Y}{V} = 2 k^2 Y, \\
  \\
\Gm{U}{U}{Z} = \Gm{Z}{U}{V} = \Gm{U}{Z}{V} = - 2k^2 Z.
\ea
\label{2.22.4}
\ee

\nit
-- The only non-vanishing covariant components of the curvature are 

\be
R_{UYUY}\, =\, - R_{UZUZ}\, =\, -2 k^2. 
\label{2.22.5}
\ee

\nit
Thus in these coordinates the curvature components are constant inside the 
wave, and we conclude that our particular planar wave solution is actually 
like a blockwave: at the boundaries $U = 0$, $U = -L$ the curvature 
components jump from zero to the values (\ref{2.22.5}) and back to zero, 
whilst in between they are constant. This makes it easy to visualize how our 
particular solution (\ref{2.16}) can be used to construct general planar 
wave solutions with polarization along the $Y$- and $Z$-axes: essentially 
it amounts to glueing together sufficiently narrow block waves of fixed 
curvature to obtain solutions in which the curvature components vary 
according to some arbitrary  profile.

The result (\ref{2.22.5}) also allows one to verify once more by a one-line
computation that the Ricci tensor vanishes identically for these planar-wave 
geometries. 
\vs

\nit
With these results in hand, our next aim is to establish the relation
between the flat half-spaces before and after the wave. We have already 
observed that the origin $x = y = z = 0$ becomes the origin $X = Y = Z = 0$ 
for all times $t$ or $T$, respectively. Next observe, that the coordinate 
transformation (\ref{2.20}) is not a Lorentz transformation: the coordinates 
$(t,x,y,z)$, defining an inertial frame before the passage of the wave,  
represent a non-inertial frame after passage. As a check, note that the 
jacobian of the transformation is

\be
\left| \dd{X^{\mu}}{x^{\nu}} \right|\, =\, fg\, \neq 1, 
  \hspace{2em} \mbox{for}\, \xi =  ct - x  \neq 0.
\label{2.22.6}
\ee

\nit
Indeed, a system of synchronized, equidistant clocks at rest in the first 
coordinate system, which operationally defines an inertial frame before the 
wave arrives, is neither synchronized nor equidistant in the final inertial 
frame. Moreover, in general it cannot be made so by a simple Lorentz 
transformation: the clocks have been accelerated with respect to each other 
by the wave, and ultimately define a non-inertial frame at late times. This 
is verified by the explicit calculation of geodesics in the next section.   

From this analysis it will be clear, that in principle it is possible to
determine the passage, and measure the characteristics, of a planar 
gravitational wave by measuring the acceleration it imparts to test masses 
in the laboratory. Indeed, such measurements can determine the functions 
$(\Lb,f,g)$ from the relation between $(t,x,y,z)$ and $(T,X,Y,Z)$. Although
in this form the statement holds only for waves of the type discussed, the 
principles for other types of waves are the same, even if the functions 
characterizing the relation between the initial and final Minkowski spaces 
are generally different. 

\section{Scattering of test particles}{\label{S3.4}}

In order to study the response of test masses to passing gravitational 
waves, it is necessary to solve for the geodesics of space-time in the 
gravitational field generated by the wave. We are particularly interested 
in the worldlines of particles initially at rest in a specific inertial 
frame (the laboratory). Observing their motion in the final inertial 
frame gives the scattering data, from which the properties of the 
gravitational wave can then be inferred relatively easily.  

In principle it is very easy to find geodesics: they correspond to the 
worldlines of particles in free fall. Consider therefore a particle at rest 
in the initial Minkowski frame; its four co-ordinates are 

\be
x^{\mu}(\tau)\, =\, (c\tau, \xi_1, \xi_2, \xi_3),
\label{2.24}
\ee

\nit
where the three vector {\boldmath $\xi$} = $(\xi_1,\xi_2,\xi_3)$ fixing the 
position of the particle is constant; note also that by definition for a 
particle at rest in an inertial frame the co-ordinate time equals the proper 
time $\tau$. 

In the co-ordinate system we use, a particle with co-ordinates (\ref{2.24})
is actually always in free fall, its co-ordinates in the $x^{\mu}$-frame 
do not change if it enters a non-trivial gravitational field. Of course, in 
an arbitrary gravitational field the $x^{\mu}$-frame is not an inertial frame,
and even if at late times space-time is flat again the particle will have 
acquired a finite, generally non-vanishing four velocity. However, its 
position in the final Minkowski frame can be found straightforwardly by 
applying the co-ordinate transformation (\ref{2.20}). 
 
Let us first confirm the above statements by a simple mathematical argument.
Then we turn to apply the result to find the actual motion of the test particle
in the final Minkowski frame. We begin by noting that in the $x^{\mu}$-frame
the metric for the gravitational wave is always of the form (\ref{2.1}), and 
therefore the only non-vanishing components of the connection are those given 
in eq.(\ref{2.3}). In particular, in the $x^{\mu}$-frame the components 
$\Gm{0}{0}{\mu}$ always vanish. 

On the other hand, for a particle with the worldline (\ref{2.24}), the
four velocity is purely time-like and constant:

\be
u^{\mu}\, =\, \frac{dx^{\mu}}{d\tau}\, =\, (c, 0, 0, 0).
\label{2.25}
\ee

\nit
Then the four acceleration in this frame vanishes identically, as does the
gravitational force: 

\be
\Gm{\nu}{\lb}{\mu}\, u^{\nu} u^{\lb}\, =\, 0.
\label{2.26}
\ee

\nit
As a result the geodesic equation (\ref{1.6}) is satisfied, proving that
(\ref{2.24}) represents the worldline of a particle at {\em all} times. 
\vspace{2ex}

\nit
What we are particularly interested in, is the position and velocity
of the particle at the moment it comes out of the gravitational wave. 
It has already been remarked that the origin {\boldmath $\xi$} = {\bf 0} 
remains at rest and coincides with the origin of the final Minkowski frame. 
Therefore at late times the origin has laboratory coordinates 

\be
X^{\mu}_0 (\tau)\, =\, \lh c\tau, 0, 0, 0 \rh.
\label{2.27}
\ee

\nit
Let us compare this with the four co-ordinates of a particle away from the
origin in the $(y,z)$-plane: {\boldmath $\xi$} = $(0, \xi_2, \xi_3) \neq$ 
{\bf 0}. For such a particle the values of the metric components at late 
times are

\be
\ba{cc}
       \ba{lll}
       f(0,\tau) & = & a\, -\, p c \tau, \\
       g(0,\tau) & = & b\, -\, q c \tau, 
       \ea &
               c\tau \geq L.
\ea
\label{2.28}
\ee

\nit
Here $(a,b;p,q)$ have the values quoted before, eq.(\ref{2.18}). For $\Lb$ 
one finds in the same domain $c\tau \geq L$:

\be
\Lb\, =\, a p \xi_2^2\, +\, b q \xi_3^2\, -\, 
          \lh p^2 \xi_2^2 + q^2 \xi_3^2 \rh\, c \tau.
\label{2.29}
\ee

\nit
As a result, the Minkowski co-odinates of this particle at late proper times
are

\be
X^{\mu}_1 (\tau)\, =\, \lh c T_1, X_1, Y_1, Z_1 \rh,
\label{2.30}
\ee

\nit
with

\be
\ba{lll}
c\,T_1 & = & \dsp{ - \frac{1}{2}\, \lh a p \xi_2^2 + b q \xi_3^2 \rh\, +\, 
    \frac{c\tau}{2}\, \lh 2 +  p^2 \xi_2^2 + q^2 \xi_3^2 \rh, }\\
 & & \\
X_1 & = & \dsp{ - \frac{1}{2}\, \lh a p \xi_2^2 + b q \xi_3^2 \rh\, +\, 
      \frac{c\tau}{2}\, \lh p^2 \xi_2^2 + q^2 \xi_3^2 \rh, }\\
 & & \\
Y_1 & = & a \xi_2\, -\, p \xi_2 c \tau, \\
 & & \\
Z_1 & = & b \xi_3\, -\, q \xi_3 c \tau. \\
\ea
\label{2.31}
\ee

\nit
Note, that clocks which were originally synchronized ---same value of $t = 
\tau$ at early proper time--- are no longer so after passage of the 
gravitational wave: $T_1$ is not equal to $T_0 = \tau$ at late proper time. 
Before we can calculate the position of the test particle at synchronized 
co-ordinate time $T = \tau$, in the final Minkowski frame, we first have to 
correct for this gravitationally induced position-dependent time shift. 

To determine the instantaneous proper distance between the particle
with worldine $X^{\mu}_1(\tau)$ and the origin, we have to ask at what 
proper time $\bar{\tau}$ the time co-ordinate $T_1$ equals the time $T_0$ 
measured by a clock at rest in the origin:

\be
T_1(\bar{\tau})\, =\, \tau,
\label{2.32}
\ee

\nit
with the result 

\be
c\bar{\tau}\, =\, \frac{2c\tau + ap \xi_2^2 + bq \xi_3^2}{2 + p^2\xi_2^2 +
                  q^2 \xi_3^2}.
\label{2.33}
\ee

\nit
The position at this proper time, $\bar{X}^{\mu}_1 = X^{\mu}_1(\bar{\tau})$,
can now be evaluated:

\be
\ba{lll}
\bar{X}_1 & = & \dsp{ \frac{-\lh ap \xi_2^2 + bq \xi_3^2\rh + c\tau
   \lh p^2 \xi_2^2 + q^2 \xi_3^2 \rh }{2  + p^2\xi_2^2 + q^2 \xi_3^2}, }\\
 & & \\
\bar{Y}_1 & = & \dsp{ \xi_2\, \lh \frac{\lh aq - bp \rh q \xi_3^2 + 
   2 \lh a - pc \tau \rh}{2 + p^2 \xi_2^2 + q^2 \xi_3^2} \rh, }\\
 & & \\
\bar{Z}_1 & = & \dsp{ \xi_3\, \lh \frac{-\lh aq - bp \rh p \xi_2^2 +
   2 \lh b - qc \tau \rh}{2 + p^2 \xi_2^2 + q^2 \xi_3^2} \rh, }
\ea
\label{2.34}
\ee

\nit
Finally we can also determine the velocity of the test particle:

\be
\frac{\mbox{\boldmath{$v$}}}{c}\, =\, \frac{1}{2+ p^2 \xi_2^2 + q^2 \xi_3^2}\,
  \lh p^2 \xi_2^2 + q^2 \xi_3^2, - 2p \xi_2, -2q \xi_3 \rh,
\label{2.36} 
\ee 

\nit
and as a result the kinetic energy is 

\be
\frac{1}{2}\, M \mbox{\boldmath{$v$}}^2\, =\, Mc^2\, \frac{\lh p^2 \xi_2^2 + 
 q^2 \xi_3^2 \rh\, \lh 4 + p^2 \xi_2^2 + q^2 \xi_3^2 \rh}{
 \lh 2 + p^2 \xi_2^2 + q^2 \xi_3^2 \rh^2}.
\label{2.37}
\ee

\nit
From this analysis we draw the conclusion, that not only in general test 
particles are accelerated by the gravitational wave, but also that the 
acceleration and hence the final velocity depend on the position of the 
particle. Therefore no Lorentz transformation with any fixed boost velocity 
$v$ can bring all test particles initially at rest w.r.t.\ one another back 
to rest simultaneously after passage of the wave. This result explicitly 
demonstrates the inequivalence of the initial and final Minkowski 
space-times.

\section{General planar waves} 

Having studied in great detail a very specific planar wave solution of the 
Einstein equations, we now briefly consider the general planar wave solution 
defined by metrics of the form (\ref{2.22}): 

\be
ds^2\, =\, - 2 dUdV\, -\, 2 K(U,Y,Z) dU^2\, +\, dY^2\, +\, dZ^2.
\label{n1.0}
\ee

\nit
It was mentioned below eq.(\ref{2.22.5}) that solutions of this type can be 
found by glueing together block waves of constant curvature. The general 
solution is obtained analytically by allowing for arbitrary dependence of 
$K(U,Y,Z)$ on its arguments. The expressions for the corresponding connection 
components are  

\be
\Gm{U}{U}{V} = K_{,U}, \hspace{2em} \Gm{Y}{U}{V} = \Gm{U}{U}{Y} = K_{,Y},
 \hspace{2em} \Gm{Z}{U}{V} = \Gm{U}{U}{Z} = K_{,Z},
\label{n1.1}
\ee

\nit
all others being zero. Up to permutation of indices, the only non-vanishing 
components of the Riemann curvature tensor then turn out to be 

\be 
\ba{l}
R_{UYUY}\, =\, - K_{,YY}, \hspace{3em} R_{UZUZ}\, =\, - K_{,ZZ}, \\
 \\
R_{UYUZ}\, =\, R_{UZUY}\, =\, - K_{,YZ}.
\ea 
\label{n1.2}
\ee

\nit
As a result the Ricci tensor takes the simple form 

\be
R_{MN}\, =\, R_{UU}\, \del_{M}^{U} \del_{N}^{U},
\label{n1.3}
\ee

\nit
with 

\be
R_{UU}\, =\, - \lh K_{,YY} + K_{,ZZ} \rh\, =\, - \Del_{trans} K. 
\label{n1.4}
\ee

\nit
Here $\Del_{trans}$ denotes the laplacian in the transverse $Y$-$Z$-plane.  
It is convenient to introduce complex co-ordinates in this plane:

\be
\zg = \lh Y + i Z \rh/\sqrt{2}, \hspace{3em} \bzg = \lh Y - iZ \rh/\sqrt{2}.
\label{n2.4}
\ee

\nit
The Einstein equations in empty space-time then reduce to the linear second 
order wave equation for $K$: 

\be
- \Del_{trans} K\, = - K_{,\bzg \zg}\, =\, 0,
\label{n3.4}
\ee

\nit 
The general solution of this equation is a sum of holomorphic and 
anti-holomorphic functions of $(\zg, \bzg)$. Expanding in Fourier modes 
it can be written as 

\be
K_0(U,\zg,\bzg)\, =\, \sum_{n=0}^{\infty}\, \int_{-\infty}^{\infty} 
  \frac{dk}{2\sqrt{\pi}}\, \lh \ve_n(k) e^{-ikU} \zg^n + 
  \bar{\ve}_n(k) e^{ikU} \bzg^n \rh.
\label{n1.5}
\ee

\nit 
From eqs.(\ref{n1.2}) it follows that the constant and linear terms in $\zg$
and $\bzg$ correspond to a vanishing Riemann curvature tensor and hence 
describe flat space-time. Therefore it should always be possible to find a 
coordinate system in which these terms are absent. In this system the 
expansion (\ref{n1.5}) in Fourier modes then starts at $n = 2$. 

The proper-time equations of motion for a point mass take the form 

\be
\ba{ll}
\dsp{ \frac{d^2U}{d\tau^2}\, =\, 0, } & \dsp{ \frac{d^2V}{d\tau^2}\, =\, 
      -\, \gam^2 K_{,U}\, -\, 2\gam \frac{dY}{d\tau}\, K_{,Y}\,
      -\, 2\gam \frac{dZ}{d\tau}\, K_{,Z}, } \\  
 & \\  
\dsp{ \frac{d^2Y}{d\tau^2}\, =\, -\, \gam^2 K_{,Y}, } & 
      \dsp{ \frac{d^2Z}{d\tau^2}\, =\, -\, \gam^2 K_{,Z}. }\\ 
\ea
\label{n1.6}
\ee

\nit
Here we have already inserted the conservation law for the proper $U$-velocity 

\be
\frac{dU}{d\tau}\, \equiv\, \gam\, =\, \mbox{constant.}
\label{n1.7}
\ee

\nit  
The origin of proper time can be chosen on the light-cone $U(0) = 0$, 
with the result that $ U = \gam \tau$. It is then possible to exchange 
the proper-time $\tau$ for the light-cone time $U$, which sometimes 
leads to simplifications. Next, the conservation law for the particle 
hamiltonian, generating time-like geodesic flow, gives 

\be
\gam \frac{dV}{d\tau}\, +\, \gam^2 K\, =\, \frac{1}{2}\, 
    \lh \lh \frac{dY}{d\tau} \rh^2 + \lh \frac{dZ}{d\tau} \rh^2 + 
    c^2 \rh. 
\label{n1.8}
\ee

\nit
We can combine the last two equations to find equivalent expressions 
for the proper-time derivatives of $(T,X)$. Adding the square of the 
$X$-component of the proper velocity to the left- and right-hand side 
of eq.(\ref{n1.8}) gives

\be 
\ba{lll}
\dsp{ \frac{c^2}{2}\, \lh \frac{dT}{d\tau} \rh^2 } & = & \dsp{ 
  \frac{1}{2}\, \lh \sqrt{2}\, \gam + \frac{dX}{d\tau} \rh^2 } \\
 & & \\
 & = & \dsp{ \frac{1}{2}\, \lh c^2 + \lh 
       \frac{d \mbox{\boldmath$R$}}{d\tau} \rh^2 \rh\, -\, 
       \gam^2 K. } 
\ea
\label{n1.9}
\ee 

\nit 
Defining the velocity in the laboratory frame as {\boldmath $v$} = 
$d${\boldmath $R$}/$dT$, eq.(\ref{n1.9}) leads to the result 

\be
\frac{dT}{d\tau}\, =\, \sqrt{ \frac{1 - 2 \gam^2 K/c^2}{1 - 
   \mbox{\boldmath $v$}^2/c^2} }.
\label{n1.10}
\ee

\nit 
This establishes the physical interpretation of $K$ as the 
gravitational potential determining the gravitational contribution 
to the time-dilation (redshift). We can invert this relation to 
establish an expression for the constant $\gam$ in terms of the 
gravitational potential $K$ and the velocity components:

\be
\frac{\gam}{c}\, \sqrt{2}\, =\,  \frac{dT}{d\tau}\, \lh 1 - 
  \frac{v_x}{c} \rh\, =\, \frac{1}{\sqrt{ \dsp{\frac{1 - \mbox{
  \boldmath $v$}^2/c^2}{(1 - v_x/c)^2} }\, + K }}. 
\label{n1.11}
\ee

\nit
An immediate corrolary of this result is that the quantity 

\be
h\, =\, K\, +\, \frac{1 - \mbox{\boldmath $v$}^2/c^2}{(1 - v_x/c)^2}  
\label{n1.12}
\ee

\nit
is a constant of motion. This result takes the place of conservation 
of energy for test particles in the field of the gravitational wave. 
It results from the light-cone co-ordinate $V$ being cyclic.   

Thus the equations for $(U,V)$ can be integrated in general for arbitrary 
$K(U,Y,Z)$. Then it only remains to solve the equations for $(Y,Z)$ on the 
second line of eq.(\ref{n1.6}). Of course, the explicit solutions of these 
equations depend on the specific form of $K(U,Y,Z)$. 

\section{The gravitational field of a light wave} 

So far we have considered gravitational waves in empty space-time. But 
in nature gravitational waves will most likely be associated with other 
physical phenomena, with the dynamical behaviour of matter and energy. 
In fact we expect gravitational waves to accompany almost any time-varying 
distributions of matter and energy, provided the motions are not too trivial 
(like uniform acceleration). 

In this respect is instructive to study a relative simple and well-known 
process, which is nevertheless quite non-trivial: the propagation of 
electro-magnetic waves. Waves in the electro-magnetic field provide an 
example of a time-varying energy and momentum distribution in space-time, 
accompanied by a co-traveling gravitational wave field. The physical 
presence of this gravitational field traveling at the speed of light can 
be demonstrated in principle by considering the motion of an electrically 
neutral point-like test particle. Although it is totally insensitive to 
the electro-magnetic wave, it does feel the associated gravitational wave 
and will therefore start to oscillate. These orbits of neutral point-masses 
are quite non-trivial; in general they are non-periodic, except for the 
case of zero-frequency: a pair of constant crossed electric and magnetic 
fields generates pure harmonic motion of a neutral point mass by its 
accompanying gravitational field. This is a quite unexpected and strange 
phenomenon, which may best be compared with the Josephson effect in 
superconductivity, in which a constant potential generates an oscillating 
current. In fact we will demonstate an even closer analogy in the case of 
scalar fields in the next section. 

With the conventional energy-momentum tensor for the electro-magnetic field, 
the Einstein-Maxwell equations describing the coupling between gravity 
and electro-magnetism read \ct{AE1}

\be
R_{\mu\nu}\, =\, - \frac{8 \pi \ve_0 G}{c^2}\, \lh F_{\mu\lb} 
    F_{\nu}^{\:\:\lb} - \frac{1}{4} g_{\mu\nu} F^2 \rh,
\label{1}
\ee

\nit
and

\be
D_{\mu} F^{\mu\nu}\, =\, 0.
\label{2}
\ee

\nit
Because the energy-momentum tensor of the electro-magnetic field is traceless, 
the first equation implies that the scalar curvature vanishes, $R = 0$. 

A free monochromatic plane electromagnetic wave of angular frequency 
$\og = kc$ and traveling in the $x$-direction is described in the Coulomb 
gauge by a vector potential 

\be
\vec{A}\, =\, \vec{a} \sin k(x - ct)),
\label{n.1}
\ee

\nit
where $\vec{a}$ is a constant vector in the $y$-$z$-plane: $a_x = 0$. The 
corresponding electric and magnetic fields are

\be
\vec{E}\, =\, - \dd{\vec{A}}{t}\, =\, \og \vec{a}\, \cos k(x - ct), \hspace{2em}
\vec{B}\, =\, \vec{\nabla} \times \vec{A}\, =\, \vec{k} \times \vec{a}\, 
  \cos k(x - ct).
\label{n.2}
\ee

\nit
The wave-vector $\vec{k} = (k,0,0)$ is orthogonal to $\vec{a}$, hence $\left| 
\vec{k} \times \vec{a} \right| = \left| k \vec{a} \right| = ka$, and

\be
\left| \vec{E}\right| = \left| c \vec{B} \right| = E_0 \cos k(x - ct), 
\hspace{3em} E_0\, =\, \og a,
\label{n.3}
\ee

\nit
whilst $\vec{E} \cdot \vec{B} = 0$. The wave (\ref{n.1}) remains a solution 
in general relativity provided the covariant derivative in eq.(\ref{2}) acts 
as an ordinary derivative. Now from the symmetry of the Riemann-Christoffel 
connection $\Gam_{\mu\nu}^{\:\:\:\:\:\lb} = \Gam_{\nu\mu}^{\:\:\:\:\:\lb}$ 
and the anti-symmetry of the electro-magnetic field-strength tensor 
$F^{\mu\nu} = - F^{\nu\mu}$ it follows that the covariant divergence of 
eq.(\ref{2}) can be written explicitly as

\be
D_{\mu} F^{\mu\nu}\, =\, \pl_{\mu} F^{\mu\nu}\, +\,  
    \Gam_{\lb\mu}^{\:\:\:\:\:\mu} F^{\lb\nu}\, =\, 0.
\label{n.4}
\ee

\nit
Therefore the covariant derivative turns into an ordinary derivative if
the contracted connection vanishes: $\Gam_{\lb\mu}^{\:\:\:\:\:\mu} = 0$.
This happens if the metric satisfies $g = \det g_{\mu\nu} =$ constant. 

The symmetry of the plane-wave configuration implies that the energy
momentum of the electro-magnetic field varies only in the $x$- and 
$t$-directions; thus we expect the curvature to change only in those
directions as well. Moreover, to keep the electric and magnetic components
of the wave perpendicular we require the metric in the $y$-$z$-plane to
be trivial. Finally, as the plane-wave configuration depends only on 
the variable $(ct - x)$ it is convenient to switch to light-cone 
coordinates 

\be
u\, =\, \frac{ct - x}{\sqrt{2}}, \hspace{3em} 
v\, =\, \frac{ct + x}{\sqrt{2}}.
\label{n.5}
\ee 

\nit
The above requirements can be satisfied by taking a metric of the form 

\be
ds^2\, =\, - 2 du dv\, -\, 2 K(u,y,z) du^2\, +\, dy^2\, +\, dz^2.
\label{n.6}
\ee

\nit
This {\em Ansatz} for the metric is the same as that for free gravitational 
waves, eqs.(\ref{2.22}), (\ref{n1.0}). It has constant determinant $g = -1$ 
and is manifestly flat in the transverse plane. 

The non-vanishing components of the Riemann-Christoffel connection are the same
as in eq.(\ref{n1.1}):

\be
\Gam_{uu}^{\:\:\:\:\:v}\, =\, K_{,u}, \hspace{2em}
\Gam_{yu}^{\:\:\:\:\:v}\, =\, \Gam_{uu}^{\:\:\:\:\:y}\, =\, 
  K_{,y}, \hspace{2em} 
 \Gam_{zu}^{\:\:\:\:\:v}\, =\, \Gam_{uu}^{\:\:\:\:\:z}\, =\, 
  K_{,z}.
\label{n.7}
\ee

\nit
From these expressions one can explicitly verify that the contracted form of 
the connection vanishes: $ \Gam_{\lb\mu}^{\:\:\:\:\:\mu} = 0$; this implies
that Maxwell's equations are satisfied indeed. 

As before, the non-zero components of the Riemann curvature are 

\be 
\ba{l}
R_{yuyu}\, =\, - K_{,yy}, \hspace{3em} 
R_{zuzu}\, =\, - K_{,zz}, \\
 \\
R_{yuzu}\, =\, R_{zuyu}\, =\, - K_{,yz}.
\ea
\label{n.9.1}
\ee

\nit 
Then the Ricci tensor reads 

\be
R_{\mu\nu}\, =\, R_{uu}\, \del_{\mu}^u \del_{\nu}^u,
\label{n.10}
\ee

\nit
where again 

\be
R_{uu}\, =\, -\, \lh K_{,yy} + K_{,zz} \rh.
\label{n.11}
\ee

\nit
From eq.(\ref{n.2}), the energy-momentum tensor of the electro-magnetic wave 
takes the form 

\be
 F_{\mu\lb} F_{\nu}^{\:\:\lb} - \frac{1}{4} g_{\mu\nu} F_{\kg\lb}^2\, =\,
 \lh F_{ux}^2 + F_{uy}^2 \rh\, \del_{\mu}^u \del_{\nu}^u\, =\, 2 k^2 
 \vec{a}^{\, 2}\, \cos^2 \lh \sqrt{2} k u\rh\, \del_{\mu}^u \del_{\nu}^u, 
\label{n.8}
\ee

\nit
with 

\be
F_{ui}\, =\, A_{i,u}\, =\, - \frac{1}{c\sqrt{2}}\, \lh E_i + 
  \eps_{ij} cB_j \rh\, =\, \sqrt{2}\, k a_i\, \cos \sqrt{2} k u,
\label{n.9}
\ee

\nit
with $\eps_{ij}$ the 2-dimensional anti-symmetric epsilon symbol 
in the transverse $(y,z)$-plane. 
 
Comparing eqs.(\ref{n.8}) and (\ref{n.10}), and introducing as in 
eq.(\ref{n2.4}) the complex coordinates $\zg = \lh y + i yz \rh/\sqrt{2}$ 
and $\bzg = \lh y - iz \rh / \sqrt{2}$, we see that they match indeed 
provided the single condition: 

\be
K_{,\bzg \zg}\, =\, \frac{4 \pi \ve_0 G}{c^4}\, \lh \vec{E}^{\,2} + 
   c^2 \vec{B}^{\,2} \rh\, =\, \frac{8 \pi \ve_0 G}{c^4}\,E_0^2\, 
   \cos^2 \sqrt{2} k u ,
\label{n.12}
\ee

\nit
is satisfied. Remarkably, this equation is linear in the metric component $K$.
Therefore its general solution can be given as 

\be
K(u,y,z)\, =\, \frac{8 \pi \ve_0 G}{c^4}\,  \bzg \zg\, E_0^2\, 
 \cos^2 \lh\sqrt{2} k u\rh\, +\, f(u;\zg)\, +\, \bar{f}(u;\bzg),
\label{n.13}
\ee

\nit
where the first term on the right is a special solution of the inhomogeneous 
Einstein equation, whilst $f(u;\zg)$ is an arbitrary complex analytic function 
of $u$ and $\zg$, representing the general solution of the homogeneous equation
\ct{KSMH2}. Thus the general solution of Einstein's equations is seen to be a 
superposition of a special gravitational wave, generated by the energy-momentum 
of the electro-magnetic field, and an arbitrary free planar gravitational wave 
traveling in the same direction. 

It is straightforward to extend the solution to the case of a pulse of 
radiation described by a vector potential 

\be
\vec{A}(x,t)\, =\, \int dk\, \vec{a}_k\, \sin k(x - ct),
\label{nn.1}
\ee

\nit
where the direction of polarization determined by $\vec{a}_k$ may depend on 
$k$ provided it is transverse to the axis of propagation: $\vec{k} \cdot 
\vec{a}_k = 0$. The energy momentum tensor of the pulse is similar to that of 
the monochromatic wave (\ref{n.8}):

\be \ba{l}
\dsp{ F_{\mu\lb} F_{\nu}^{\:\:\lb} - \frac{1}{4} g_{\mu\nu} F_{\kg\lb}^2\, 
 =\, \lh F_{ux}^2 + F_{uy}^2 \rh\, \del_{\mu}^u \del_{\nu}^u }\\
  \\ 
 \dsp{\hspace {1em} =\, \del_{\mu}^u \del_{\nu}^u\, \frac{1}{c^2}\, 
 \int dk \int dq\, \vec{E}_k \cdot \vec{E}_q\, 
 \lh \cos \sqrt{2} (k + q) u\, +\, \cos \sqrt{2} (k - q) u \rh. }
\ea
\label{nn.2}
\ee

\nit
The corresponding metric is again of the form (\ref{n.6}), with

\be 
\ba{l}
K(u,\zg, \bzg)\, =\, K_0(u,\zg,\bzg)\, +      \\
 \\
 \hspace{1em} \dsp{ +\, \frac{4 \pi \ve_0 G}{c^4}\, \bzg \zg 
  \int dk \int dq\, \vec{E}_k \cdot \vec{E}_q\, 
  \lh \cos \sqrt{2} (k + q) u + \cos \sqrt{2} (k - q) u \rh. }
\ea
\label{nn.3}
\ee
   
\nit
The physical nature of the special gravitational wave generated by the 
electro-magnetic field can be investigated by solving the equations 
for time-like geodesics, representing the orbits of electrically neutral 
massive test particles. Parametrizing the geodesics by the proper time 
$\tau$ and using an overdot to denote proper-time derivatives, the  
geodesic equation is 

\be
\ddot{x}^{\mu}\, +\, \Gam_{\nu\lb}^{\:\:\:\:\:\mu}\, \dot{x}^{\nu} 
  \dot{x}^{\lb}\, =\, 0. 
\label{n.15.0}
\ee

\nit
Consider the simplest case of a monochromatic electro-gravitational wave, with 
$f(u;\zg) = 0$; then the metric component $K$ can be written as 

\be
K_{em}(u,x,y)\, =\, \frac{\Og_0^2}{2}\, \lh 1 + \cos 2\sqrt{2} ku \rh\, 
  \lh y^2 + z^2 \rh.
\label{n.15.1}
\ee

\nit
In this expression we have defined the constant

\be
\Og_0^2\, =\, \frac{4\pi \ve_0 G}{c^4}\, E_0^2.
\label{n.15.2}
\ee

\nit
Using this in the connections (\ref{n.7}), the first geodesic equation 
for $u(\tau)$ becomes 

\be
\ddot{u}\, =\, 0.
\label{n15.3}
\ee

\nit
It follows that the momentum $\dot{u}$ is a constant of motion:

\be
\dot{u}\, =\, \gam.
\label{n.15.4}
\ee

\nit  
In addition we can write down two other constants of motion.
The first one is the hamiltonian 

\be
H\, =\, \frac{m}{2}\, g_{\mu\nu}\, \dot{x}^{\mu} \dot{x}^{\nu}\, 
    =\, -\, \frac{mc^2}{2},
\label{n.16}
\ee

\nit
where we have used that for time-like geodesics the geodesic interval
is measured by proper time: $ds^2 = -c^2 d\tau^2$. From the expression 
for the metric in eq.(\ref{n.6}) it then follows that 

\be
\dot{v}\, =\, \frac{1}{2\gam}\, \lh c^2 + \dot{y}^2 + \dot{z}^2\rh\, 
                    - \, \gam K. 
\label{n.18}
\ee

\nit
The other constant of motion is the angular momentum in the $z$-direction  

\be
J\, =\, y \dot{z}\, -\, z \dot{y}.
\label{n.17}
\ee

\nit 
It remains to solve for $y(\tau)$ and $z(\tau)$. The geodesic equations
for these coordinates take the form 

\be
\ddot{y}\, =\, -\, \frac{\og_0^2}{2}\, \lh 1 + \cos 2 \og_1 \tau \rh\, y, 
\hspace{2em}
\ddot{z}\, =\, -\, \frac{\og_0^2}{2}\, \lh 1 + \cos 2 \og_1 \tau \rh\, z,
\label{n.19}
\ee

\nit
with the frequencies $\og_0$ and $\og_1$ defined by 

\be
\og_0\, =\, \gam \Og_0 \sqrt{2}, \hspace{3em} \og_1\, =\, \gam k \sqrt{2}.
\label{n.20}
\ee

\nit
In the limit of static electric and magnetic fields, $k = \og_1 = 0$ with 
$E_0$ and $B_0$ fixed, they reduce to ordinary oscillator equations, with 
purely harmonic solutions of frequency $\og_0$. Hence we find that a neutral 
test particle in static crossed electric and magnetic fields executes a 
harmonic motion in the $y$-$z$-plane, as a result of an induced gravitational 
wave \ct{jw3}. As pointed out in the introductory remarks, this phenomenon as 
well as a similar one for the gravitational effect of a scalar field with 
constant gradient \ct{jw1,jw3}, recall the Josephson effect in superconductivity.

For $\og_1 \neq 0$ eqs.(\ref{n.19}) are particular instances of the Mathieu 
equation, the solutions of which are well-known \ct{MF}. In general they 
are not periodic. For the present application it is convenient to proceed as 
follows. Introduce the new affine parameter $\lb = \og_1 \tau$; then writing
$\eta = \og_0/\og_1$ for the ratio of the two frequencies we obtain the 
equation of motion

\be
\frac{d^2 y}{d\lb^2}\, +\, 
      \frac{1}{2}\, \eta^2\, \lh 1 + \cos 2\lb \rh\, y\, =\, 0,
\label{n.22.1}
\ee

\nit 
and a similar equation for $z(\lb)$. In practice we always have $\eta \ll 1$ therefore we can expand $y(\lb)$ in powers of $\eta^2$:

\be
y(\lb)\, =\, \sum_{n=0}^{\infty}\, c_n(\lb) \eta^{2n}.
\label{n22.2}
\ee

\nit
This can be solved recursively for the $c_n(\lb)$:

\be
\frac{d^2 c_0}{d\lb^2}\, =\, 0, \hspace{3em}
\frac{d^2 c_{n+1}}{d\lb^2}\, =\, - \frac{1}{2}\, \lh 1 + \cos 2\lb \rh\, c_n.
\label{n.23}
\ee

\nit
The solution of these equations is straightforward. We fix the constants of 
integration such that $y(0) \equiv y_0 = c_0(0)$ and $\pr{y}(0) \equiv \bg_y =
\pr{c}_0(0)$, and therefore 

\be
c_k(0)\, =\, \pr{c}_k(0)\, =\,  0, \hspace{2em} k\, =\, 1,2,...
\label{n.24}
\ee

\nit 
Here the prime is used to denote a derivative with respect to $\lb$. 
The solutions then take the form 

\be
\ba{lll}
y(\lb) & = & y_0\, a(\lb)\, +\, \bg_y\, b(\lb),  \\
 & & \\
z(\lb) & = & z_0\, a(\lb)\, +\, \bg_z\, b(\lb),
\ea
\label{n.25}
\ee

\nit
where the universal functions $a(\lb)$ and $b(\lb)$ contain all the 
dependence on the affine parameter $\lb$. They possess the expansions

\be
\ba{lll}
a(\lb) & = & \dsp{ 1\, +\, \frac{\eta^2}{4}\, a_1(\lb)\, +\, \frac{\eta^4}{16}\,
  a_2(\lb)\, +\, ... } \\
 & & \\
b(\lb) & = & \dsp{ \lb \lh 1\, +\, \frac{\eta^2}{4}\, b_1(\lb)\, +\,   
  \frac{\eta^4}{16}\, b_2(\lb)\, +\, ....  \rh, }
\ea 
\label{n.26}
\ee

\nit
with 

\be
\ba{lll} 
a_1(\lb) & = & \dsp{ -\frac{1}{2}\, - \lb^2\, +\, \frac{1}{2}\, \cos 2 \lb, }\\
 & & \\
a_2(\lb) & =& \dsp{ - \frac{25}{32}\, +\, \frac{\lb^2}{4}\, +\, \frac{\lb^4}{6}\, 
              +\, \lh \frac{3}{4}\, -\, \frac{\lb^2}{2} \rh \cos 2 \lb\, 
              +\, \lb\, \sin 2 \lb\, +\, \frac{1}{32}\, \cos 4 \lb, } \\ 
 & & \\ 
b_1(\lb) & = & \dsp{ \frac{1}{2}\, - \frac{\lb^2}{3}\, - \frac{\sin   
          2\lb}{2\lb}\, +\, \frac{1}{2}\, \cos 2 \lb,   } \\ 
 & & \\  
b_2(\lb) & = & \dsp{ \frac{45}{32}\, - \, \frac{\lb^2}{4}\, +\, \frac{\lb^4}{30}\, 
         -\, \lh \frac{5}{2}\, +\, \lb^2 \rh\, \frac{\sin 2 \lb}{2\lb}\, 
         +\, \lh \frac{5}{4}\, - \, \frac{\lb^2}{6}\rh\, \cos 2 \lb } \\
 & & \\
 & & \dsp{  -\, \frac{3 }{16}\, \frac{\sin 4\lb}{4 \lb}\, +\, 
     \frac{1}{32}\, \cos 4 \lb.  } \\
\ea
\label{n.26.1}
\ee

\nit
A non-trivial check on this result follows from the conservation of 
the $x$-component of angular momentum. Its value is fixed by the initial 
positions and velocities as 

\be
J\, =\, y_0 v_z\, -\, z_0 v_y ,
\label{n.27}
\ee

\nit 
where $v_i = \og_1 \bg_i$. It is constant because the functions $a(\lb)$ and 
$b(\lb)$ satisfy the relation 

\be 
a\, \pr{b}\, -\, b\, \pr{a}\, =\, 1 .  
\label{n.27.1}
\ee

\nit
This may be checked order by order in powers of $\eta^2$. In particular, one 
finds

\be
\ba{c} 
a_1\, -\, \lb \pr{a}_1\, +\, b_1\, +\, \lb \pr{b}_1\, =\, 0, \\
 \\
\dsp{ a_2\, -\, \lb \pr{a}_2\, +\, b_2\, +\, \lb \pr{b}_2\, +\,  
   a_1 b_1 + \lb\, \lh a_1 \pr{b}_1 - b_1 \pr{a}_1 \rh\, =\, 0. }
\ea
\label{n.27.2}
\ee
 
\nit
Thus the conservation of angular momentum relates the functions $a(\lb)$ 
and $b(\lb)$. 

The expansion (\ref{n22.2}) assumes $\eta < 1$. From the explicit results 
for $a(\lb)$ and $b(\lb)$ we can infer that the coefficients remain small 
for values of $\lb$ such that $\lb \eta = \og_0 \tau < 1$, i.e.\ for
proper times $\tau < 1/\og_0$. Numerically 
 
\be
\og_0\,(\mbox{rad/sec})\, =\, 0.29 \times 10^{-18}\, \frac{\gam \sqrt{2}}{c}\, 
     E_{0}\, (\mbox{V/m}).
\label{n.28}
\ee

\nit
For non-relativistic motion $\gam \sqrt{2} \approx c$, whilst the highest 
electric fields in the laboratory are generated by lasers, with $E_0 \sim 
10^{11}$ V/m \ct{JC}. This limits $\og_0$ in practice to values less than 
$10^{-7}$ rad/sec, and therefore almost always $\og_0 \ll \og_1$. Note that
on top of the slow oscillation we observed for the case of static (zero 
frequency) electro-magnetic fields, there is now a modulation with frequencies 
$2n \og_1$, where $n$ is an integer number, but unless $\og_1 \approx \og_0$ 
the amplitude of these oscillations is very small. 

A theoretical upper limit on the frequency $\og_0$ is provided by quantum 
electro-dynamics, as the vacuum breaks down due to electron-positron pair 
creation for values of the order \ct{HE,VW}

\be
E_{crit}\, =\, \frac{\pi m_e c^2}{e \lb_e}\, =\, 4.1 \times 10^{18} 
     \mbox{V/m}.
\label{n.29}
\ee

\nit
Here $m_e$ is the electron mass, and $\lb_e$ its reduced Compton wave length;
for details we refer to ref.\ct{GMR}. The critical field strength corresponds 
to a frequency upper limit of $\og_0 \approx 1$ rad/sec. 

From the solution (\ref{n.25}) of the equations of motion it follows that a 
point mass at rest in the origin remains at rest at all times. Now clearly,
the choice of origin in the $y$-$z$-plane is arbitrary due to translation 
invariance. Therefore the non-trivial nature of the solution becomes manifest 
only if we compare the relative motion of test particles. Fortunately, using 
one test particle initially at non-zero $(y_0, z_0)$ and one at rest in the 
origin, our solutions are seen to determine the relative acceleration between
these point masses. As a result they provide a true measure for the curvature 
of space-time generated by a light-wave. 

\section{Symmetry breaking as a source of gravitational oscillations 
         \label{S3.5}}

The planar gravitational wave solutions described earlier in this chapter 
as block-waves, arise as transition regions between flat domains of 
space-time, which are related by a coordinate transformation that cannot 
be reduced to a (linear) Lorentz transformation. We have therefore 
interpreted them as domain boundaries between regions of space-time 
trapped in inequivalent classical vacua of the gravitational field 
(in the absence of a cosmological constant). This is possible because 
flat space (zero curvature) is associated with a value of the 
gravitational field, the metric $g_{\mu\nu}$, which in the appropriate 
Minkowskian coordinate system (`Minkowski gauge') is constant, 
non-vanishing and Lorentz-invariant, but not invariant under general 
coordinate transformations. In this sense the general coordinate 
invariance of the Einstein equations is broken spontaneously by the 
vacuum solutions representing flat  Minkowski space-time. 

A domain structure arising from the presence of degenerate but inequivalent 
classical vacua is a well-known consequence of spontaneous symmetry breaking 
in scalar field theories. In this section we take up this aspect of the 
the field theory and show, that dynamical domain boundaries in scalar field 
theories (scalar-type shock waves, if one prefers) are also sources 
of planar gravitational waves of the kind analysed in detail above \ct{jw1}. 
This is another instance of the general observation that almost any 
type of dynamical situation with time-dependent mass-energy distributions 
is accompanied by gravitational fields. 

The simplest scalar field theory with a continuously degenerate set of
classical vacua is that of a complex scalar field with a `mexican hat'
type of potential, as described by the lagrangian

\be
\frac{1}{\sqrt{-g}}\, \cL\, =\, - g^{\mu\nu}\, \pl_\mu \fg^* \pl_\nu \fg\, 
 -\, \frac{\lb}{2}\, \lh \fg^* \fg - \frac{\mu^2}{\lb} \rh^2,
\label{c3.8}
\ee

\nit
In this lagrangian $\hbar c \lb$ is a dimensionless coupling constant 
and $\mu$ is an inverse length ($\mu \hbar/c$ is a mass). In the natural 
system of units in which $\hbar = c = 1$ we can take $\lb$ to be 
dimensionless and $\mu$ to represent a mass. In the following equations
one then can substitute $c = 1$ everywhere.

This lagrangian (\ref{c3.8}) is invariant under rigid $U(1)$ phase shifts 
$\fg \rightarrow e^{i\ag} \fg$, with $\ag$ constant. As a result for 
$\mu^2 > 0$ there is an infinitely degenerate set of solutions of the 
equations of motion minimizing the potential (refered to as classical 
vacua), of the form

\be
\fg\, =\, \frac{\mu}{\sqrt{\lb}}\, e^{i \th},
\label{c3.9}
\ee

\nit
with $\th$ an arbitrary real constant. Clearly the solutions themselves are
not invariant under the $U(1)$ transformations: the classical vacuum 
solutions break the $U(1)$ symmetry spontaneously. However, because of 
the $U(1)$ symmetry of the dynamics these solutions are physically 
indistinguishable, and the absolute value of $\th$ is unobservable. 
On the other hand, variations in the vacuum angle between different regions 
of space-time can have observable effects \ct{Gold,NJL}. 

Parametrizing the complex scalar field as $\fg(x) = \rg(x) 
e^{i\th(x)}/\sqrt{2}$, the lagrangian becomes

\be
\frac{1}{\sqrt{-g}}\, \cL\, =\, - \frac{1}{2}\, g^{\mu\nu} \pl_\mu \rg 
  \pl_\nu \rg\, -\, \frac{\lb}{8}\, \lh \rg^2 - \frac{2\mu^2}{\lb} \rh^2\,
  -\, \frac{1}{2}\, \rg^2\, g^{\mu\nu} \pl_\mu \th \pl_\nu \th. 
\label{c3.10}
\ee

\nit
This shows that in the spontaneously broken mode of the $U(1)$ symmetry 
the theory desribes actually two real scalar fields: the field 
$\chi = \rg - \mu\sqrt{2/\lb}$, obtained by shifting $\rg$ by its classical 
vacuum value $\mu\sqrt{2/\lb}$, with a mass (or inverse coherence length) 
equal to $\mu$, which can become arbitrarily large; and the strictly 
massless field $\sg = \mu \th \sqrt{2/\lb}$, representing the Goldstone 
excitations arising from spontaneous symmetry breaking \ct{Gold,NJL}. 

Clearly at energies small compared to the scale $\mu$ set by the mass of the 
field $\chi$ the excitations of this massive field play no role and one
only has to consider the Goldstone field $\sg$, described by the effective
lagrangian 

\be
\frac{-1}{\sqrt{-g}}\, \cL\, =\, \frac{c^4}{16\pi G}\, R\, +\, 
         \frac{1}{2}\,  g^{\mu\nu} \pl_\mu \sg \pl_\nu \sg,
\label{c3.10.1}
\ee

\nit
where we have added the Einstein-Hilbert action for the gravitational 
field as this also describes a low-energy degree of freedom. Note that 
with the potential defined in eqs.(\ref{c3.8}), (\ref{c3.10}) there is no 
cosmological constant in the presence of the vacuum value of the scalar 
field, $\rg = \mu \sqrt{2/\lb}$ or equivalently $\chi = 0$.

The field equations derived from this lagrangian are the
massless 
Klein-Gordon equation for the Goldstone field $\sg$:

\be
\Box^{cov} \sg\, =\, \frac{1}{\sqrt{-g}}\, \pl_\mu \sqrt{-g}g^{\mu\nu} 
   \pl_\nu \sg\, =\, 0.
\label{c3.11}
\ee

\nit
and the Einstein-equations with a source term from the energy-momentum of
the Goldstone field:

\be
R_{\mu\nu}\, =\, - \frac{8 \pi G}{c^4}\, \pl_\mu \sg \pl_\nu \sg.
\label{c3.12}
\ee

\nit 
This system of equations admits exact planar wave solutions similar to 
those of the electro-magnetic waves discussed above. Using the same 
Ansatz (\ref{n1.0}), (\ref{n.6}) for the metric we find running 
planar gravitational waves described by a metric component $g_{uu} = 
-2 K(u,y,z)$ in combination with a scalar wave $\sg(u)$ running in the 
same direction: 

\be
\Box^{cov} \sg\, =\, \lh - 2\, \pl_u \pl_v - 2 \pl_v K \pl_v + 
  \pl_y^2 + \pl_z^2 \rh\, \sg\, =\, 0,
\label{c3.12.1}
\ee

\nit 
because both $K$ and $\sg$ are independent of $v$. 
The inhomogeneous Einstein equation now takes the form 

\be
R_{uu}\, =\, - \Del_{trans} K\, =\, -\, \frac{8 \pi G}{c^4}\, 
             \lh \pl_u \sg \rh^2,
\label{c3.12.2}
\ee

\nit
with the solution in complex transverse coordinates $(\zg, \bzg)$:

\be
K(u,y,z)\, =\, \frac{4\pi G}{c^4}\, \lh \pl_u \sg \rh^2 \bzg \zg\, +\,
               f(u;\zg)\, +\, \bar{f}(u;\bzg), 
\label{c3.12.3}
\ee

\nit
where the (anti-)holomorphic terms $K_0 = f(u;\zg) + c.c.$ denote the 
free gravitational waves that are allowed in the background. As the 
functional dependence of $\sg(u)$ on $u$ is quite general, we do not 
have to restrict ourselves to monochromatic waves, but can consider
arbitrary wave packets. 

The net effect of a scalar wave on the motion of test particles is
the same as that of an electro-magnetic wave. For the simple case of 
a monochromatic wave of wave number $k$:

\be
\sg(u)\, =\, \sg_0 \sin \sqrt{2} ku, \hspace{3em} 
\pl_u \sg(u)\, =\, k \sg_0 \sqrt{2} \cos \sqrt{2} ku, 
\label{c3.12.4}
\ee

\nit
the gravitational potential is of the form (\ref{n.15.1}) with 

\be
\Og_0\,^2 =\, \frac{4 \pi G }{c^4}\, k^2 \sg_0^2.
\label{c3.12.5}
\ee

\nit
It follows that the solutions of the equations of motion for 
a point mass in a scalar wave is also given by expressions 
(\ref{n.25})-(\ref{n.26.1}). 

In addition we also observe that scalar fields with zero frequency and 
constant gradient $\pl_u \sg(u) = 2 \mu \ag/\sqrt{\lb} $ represent a 
simple $\fg$-wave 

\be
\fg(u)\, =\, \fg_0\, e^{i\ag u \sqrt{2}}\, =\, \
  \frac{\mu}{\dsp{ \sqrt{\lb} }}\,\, e^{i\ag (x - ct)}. 
\label{c3.15}
\ee

\nit 
Such a wave can interpolate between two fixed values of the Goldstone 
field $\sg$ on a finite interval $-L \leq x - ct \leq 0$:   


\be
\ba{ll}
\sg(u)\, =\, \sg_0, & \mbox{for}\, u \leq 0; \\
 & \\
\dsp{ \sg(u)\, =\, \sg_0\, +\, \frac{2 \mu \ag u }{\sqrt{\lb}}, } & 
         \mbox{for}\, 0 \leq u \leq L/\sqrt{2};  \\
 & \\
\dsp{ \sg(u)\, =\, \sg_1\, =\, \sg_0 +\, \mu \ag L \sqrt{\frac{2}{\lb}}, } & 
         \mbox{for}\, u \geq L/\sqrt{2}.
\ea
\label{c3.13}
\ee

\nit
The wave number $\ag$ of the scalar field $\fg(u)$ is given by the 
slope of $\sg$ in eq.(\ref{c3.13}) as 

\be
\ag\, =\, \frac{\sg_1 - \sg_0}{\mu L}\, \sqrt{\frac{\lb}{2}}\, 
 \hspace{2em} \Leftrightarrow \hspace{2em}  
\frac{2 \mu \ag}{\sqrt{\lb}}\, =\, \frac{\sg_1 - \sg_0}{L/\sqrt{2}}. 
\label{c3.14}
\ee

\nit
From the geodesic equation (\ref{n.19}) with $\og_1 = 0$ we find, that 
in the scalar field with constant non-zero gradient --- in the region 
$0 \leq u \leq L/\sqrt{2}$ --- a point mass will execute a harmonic 
motion in response to the {\em gravitational} field generated by the 
uniform scalar potential difference. This response is the same as to 
the gravitational field of a uniform static electro-magnetic field. 
But here it is generated by a Goldstone field of constant growth, 
which really represents a constant change in the {\em phase} of a 
complex scalar field in the broken symmetry mode; as such the 
oscillations driving test masses through the associated gravitational 
field represent not only a mathematical, but also a physical 
analogue of the Josephson effect in superconductivity. 
% In fact on the basis of
% this argument one might expect such gravity-driven oscillations of 
% neutral particles to be possible in principle in real Josephson 
% junctions, where the phase of the Cooper-pair condensate changes 
% across the junction. In practice the frequency being proportional 
% to $G/c^4$ is far too small. 

From eqs.(\ref{c3.12.3}) and (\ref{n.9.1}) it follows that these simple 
$\fg$-waves on the finite interval $0 \leq u \leq L/\sqrt{2}$ represent 
block-waves of constant curvature

\be
R_{uyuy}\, =\, R_{uzuz}\, =\, \frac{1}{2}\, R_{uu}\, =\, 
    -\, \frac{8 \pi G}{c^4}\, \lh  \frac{\sg_1 - \sg_0}{L} \rh^2\, =\, 
    -\, \frac{16 \pi G}{c^4}\, \frac{\mu^2\ag^2}{\lb}.
\label{c3.18}
\ee

\nit
We have seen before that such block waves can be interpreted as dynamical 
gravitational domain boundaries; we observe that in this case they 
coincide with analogous domain boundaries of the scalar field. Stated 
differently, the transition between different scalar vacua also induces 
a transition between different gravitational vacua. 

The simple treatment in terms of block waves can be regularized by 
considering more sophisticated field configurations interpolating between 
different vacua; for example the regular scalar field  

\be
\sg(u)\, =\, \frac{1}{2}\, \lh \sg_1 + \sg_0 \rh\, +\, 
 \frac{(\sg_1 - \sg_0)}{\pi}\, \arctan \lh \frac{2 \pi \mu \ag} 
 {\sqrt{\lb}}\, \frac{u}{\sg_1 - \sg_0} \rh,
\label{c3.16}
\ee 

\nit
interpolates between $\sg_0$ and $\sg_1$; it also generates a smooth 
gravitational field:

\be
 R_{uyuy}\, =\, R_{uzuz}\, =\, \frac{1}{2}\, R_{uu}\, = 
  -\, \frac{16 \pi G}{c^4}\, \frac{\mu^2 \ag^2}{\lb}\,  
  \frac{1}{\dsp{ \lh 1 + \frac{\mu^2 \ag^2}{\lb}\, 
  \frac{ 4 \pi^2  u^2}{(\sg_1 - \sg_0)^2} \rh^2}}. 
\label{c3.17}
\ee 

\nit
The geodesic equations describing the motion of test masses can 
be solved analytically in closed form for this space-time geometry.
Observing that as before $\dot{u} = \gam =$ const., the equations 
of motion in the transverse plane can be written conveniently in 
terms of $u$ rather than proper time $\tau$ as affine parameter.
Then 

\be
\frac{d^2 y}{du^2}\, =\, - \frac{\og_0^2 y}{\lh 1 + \Gam^2 u^2 \rh^2},
\hspace{2em}
\frac{d^2 z}{du^2}\, =\, - \frac{\og_0^2 z}{\lh 1 + \Gam^2 u^2 \rh^2},
\label{c3.18.1}
\ee

\nit
where the parameters in the equation are given by the explicit 
expressions

\be
\og_0^2\, =\, \frac{16 \pi G}{c^4}\, \frac{\mu^2 \ag^2}{\lb}, 
 \hspace{3em}
\Gam^2\, =\, \frac{4 \pi^2 \mu^2 \ag^2}{\lb (\sg_1 - \sg_0)^2}.
\label{c3.19}
\ee

\nit
We will also define the ratio of these quantities as a new parameter

\be
\eta^2\, =\, \frac{\og_0^2}{\Gam^2}.
\label{c3.19.1}
\ee

\nit
We give the solution of the equation for $y(u)$, that of $z(u)$ 
being similar:

\be
\ba{ll}
y(u)\, = & \dsp{ 
  \sqrt{1 + \Gam^2 u^2}\, \lh y_0 \cos\lh \sqrt{1 + \eta^2} 
  \arctan \Gam u \rh\, +\, \rd }\\ 
 & \\
 & \dsp{ \ld +\, \frac{v_y}{\dsp{ \Gam \sqrt{1 + \eta^2} }}\, 
  \sin \lh  \sqrt{1 + \eta^2} \arctan \Gam u \rh \rh. }
\ea
\label{c3.20}
\ee

\nit
Here $y_0$ and $v_y$ represent the value of the $y$-coordinate and 
the velocity in the $y$-direction at $u = 0$. Note that the 
velocity at $u = \pm \infty$ is given by 

\be
\ba{lll}
\dsp{ \lim_{u \rightarrow \pm \infty}\, \frac{dy}{du} } & = &  
 \dsp{ \lim_{u \rightarrow \pm \infty}\, \frac{1}{\gam}\, \frac{dy}{d\tau} }\\ 
 & & \\ 
 & = & \dsp{ \Gam\, \lh \pm\, y_0 \cos \lh \frac{\pi}{2} 
   \sqrt{1 + \eta^2} \rh\, +\, \frac{v_y}{\dsp{ \Gam \sqrt{1 + \eta^2} }}\, 
  \sin \lh \frac{\pi}{2} \sqrt{1 + \eta^2} \rh \rh. }
\ea
\label{c3.21}
\ee

\nit
Clearly the change in proper velocity depends on the position $y_0$:

\be
\Del u_y\, =\,  \ld \frac{dy}{d\tau}\right|_{\infty}\, -\, 
  \ld \frac{dy}{d\tau}\right|_{-\infty}\,
  =\, 2 \gam \Gam\, y_0 \cos \lh \frac{\pi}{2} \sqrt{1 + \eta^2} \rh.
\label{c3.22}
\ee

\nit
From this we see once more that a system of particles at fixed 
distances and at rest w.r.t.\ each other at some early time 
$\tau_1 \rightarrow - \infty$ will be scattered by the wave and 
have all different velocities at a very late time $\tau_2 
\rightarrow \infty$: no Minkowski frame at early times remains a 
Minkowski frame at late times. This confirms our previous conclusion 
that the gravitational vacuum states, the Minkowski spaces before 
and after the wave, are inequivalent and that space-time can have 
a gravitational domain structure originating in the breaking of 
general co-ordinate invariance down to Poincar\'{e} invariance, 
in addition to a domain structure originating in broken internal 
symmetry.  



==> geod.tex <==
\chapter{Geodesics \label{C2}} 

\section{Curves and geodesics \label{S2.1}}

In this chapter we discuss how basic information about the geometry of spaces 
or space-times ---generically manifolds--- can be obtained from studying 
their geodesics. The geodesics of euclidean differentiable manifolds are 
smooth curves of stationary proper length, meaning that to first order the 
proper length of an arc does not change under small variations of the 
curve. More generally and more precisely, given a metric on a manifold 
(euclidean or lorentzian) the geodesics are those smooth curves for which 
the proper interval between any two fixed points $\cP$ and $\cP^{\prime}$ 
through which the curve passes is both well-defined and stationary. The 
interval among the fixed points can be either a maximum, a minimum or a 
saddle point.

A direct reason for geodesics to be important is that time-like geodesics 
represent the allowed trajectories of test particles in a fixed 
background space-time. But in general geodesics tell us interesting 
things about the symmetries and topology of a manifold, which often
have wider implications for physics.  

First we derive the fundamental equation characterizing geodesics. The 
proper interval $\Del s\, [\cC_{\cP \cP^{\prime}}]$ of the arc  
$\cC_{\cP\cP^{\prime}}$ of an arbitrary smooth curve $\cC$ between 
the two fixed points $(\cP,\cP^{\prime})$ is given by the integral 

\be
\Del s\, [\cC_{\cP \cP^{\prime}}] = \int_{\cC_{\cP\cP^{\prime}}} ds   
  =  \int_{\cC_{\cP\cP^{\prime}}} d \lb\, \sqrt{ \left| g_{\mu\nu} 
      \frac{dx^{\mu}}{d\lb} \frac{dx^{\nu}}{d\lb} \right| } .
\label{c2.1}
\ee

\nit
This holds for all geodesics of euclidean manifolds, and time- or 
space-like geodesics of lorentzian manifolds; $\lb$ is a continuous 
parameter on some interval of the real line, parametrizing the curve 
between the points $\cP$ and $\cP^{\prime}$ in any convenient way, 
provided the coordinates $x^{\mu}(\lb)$ of points on the curve are 
monotonic differentiable functions of this parameter: the label of any 
point must be unique and the tangent vector $\dot{x}^{\mu} = 
dx^{\mu}/d\lb$ must be well-defined. The parameter $\lb$ is then called 
an affine parameter. Note that the integral does not depend on the 
particular choice of affine parameter: it is invariant under 
differentiable changes of parametrization $\lb \rightarrow 
\lb^{\prime}(\lb)$. This freedom to choose for $\lb$ any smooth 
parametrization of the curve is often useful, but requires some care 
in interpreting results explicitly containing $\lb$. As any invariant 
geometrical results with physical interpretation can not depend on the 
choice of affine parameter, the best way to proceed is to remove any 
$\lb$-dependence from equations before drawing physical conclusions.  

The proper interval $\Del\, s [\cC_{\cP \cP^{\prime}}]$ is stationary if 
the integral does not change to first order under arbitrary smooth 
variations of the path while keeping the end points of the integral 
fixed:

\be 
\del\, \int_{\cC_{\cP\cP^{\prime}}} d \lb\, w[x(\lb)]\, =\, 0, 
\label{c2.2}
\ee

\nit
where the integrand is $w[x(\lb)] = \sqrt{ |g_{\mu\nu} \dot{x}^{\mu} 
\dot{x}^{\nu}}|$. Now after a partial integration with vanishing boundary 
terms (the end points remain fixed) the variation of the integrand can be 
written

\be 
\del w\, =\, \pm \del x^{\mu} \lh -\frac{d}{d\lb} \left[ 
             \frac{g_{\mu\nu}}{w} \frac{dx^{\nu}}{d\lb} \right]\, +\, 
             \frac{1}{2w} \dd{g_{\lb\nu}}{x^{\mu}} \frac{dx^{\lb}}{d\lb} 
             \frac{dx^{\nu}}{d\lb} \rh, 
\label{c2.2.1} 
\ee 

\nit
provided $w \neq 0$. The sign on the r.h.s.\ is positive in 
euclidean spaces or for space-like curves in lorentzian space-times, and 
negative for time-like curves in lorentzian space-times. Light-like 
curves in lorentzian space-time need special consideration, as $ds^2 = 0$ 
is equivalent to $w d\lb = 0$. 

The variational principle (\ref{c2.2}) now implies that for any smooth 
local variation $\del x^{\mu}$ the induced variation $\del w$ must 
vanish if the curve $x^{\mu}(\lb)$ is to describe a geodesic. For $w \neq 0$
we can divide the right-hand side of eq.(\ref{c2.2.1}) by $w$ once more, 
and use the fact that $w d\lb = ds$, the infinitesimal proper interval 
which is measured in the laboratory frame and independent of the choice of 
affine parameter $\lb$. We can also replace the partial derivative of the
metric in the second term by the connection; recall, that the connection 
was defined in eq.(\ref{1.5.2}) as

\be 
\Gam_{\lb\nu}^{\:\:\:\:\:\mu}\, =\, \frac{1}{2}\, g^{\mu\kg} \lh 
      \dd{g_{\lb\kg}}{x^{\nu}} + \dd{g_{\kg\nu}}{x^{\lb}} - 
      \dd{g_{\lb\nu}}{x^{\kg}} \rh.
\label{c2.2.2} 
\ee 

\nit 
This expression is actually the solution of the equation 

\be
\frac{D g_{\mu\nu}}{D x^{\lb}} = \dd{g_{\mu\nu}}{x^{\lb}} - 
  \Gm{\lb}{\mu}{\kg} g_{\kg\nu} - \Gm{\lb}{\nu}{\kg} g_{\mu\kg} = 0,
\label{c2.2.3}
\ee

\nit
stating that the metric is covariantly constant, a condition known as the 
metric postulate. From the equation above it follows that

\be
\dd{g_{\lb\nu}}{x^{\mu}}\, =\, \Gm{\mu}{\lb}{\kg} g_{\kg \nu}\, +\, 
  \Gm{\mu}{\nu}{\kg} g_{\kg \lb}.
\ee

\nit
The vanishing of $\del w$ is now seen to imply a differential equation of the 
form (1.10) for the coordinates of a point moving on the curve as a function 
of the proper interval parameter $s$: 

\be 
\frac{d^2 x^{\mu}}{ds^2}\, +\, \Gam_{\kg\nu}^{\:\:\:\:\:\mu} 
  \frac{d x^{\nu}}{ds} \frac{d x^{\kg}}{ds}\, =\, 0. 
\label{c2.3} 
\ee 

\nit 
Note, that the above procedure eliminating the affine parameter $\lb$ 
is equivalent to a choice of rate of flow of the affine parameter $d\lb$
equal to the proper interval $ds$ measured in the coordinate frame 
$\{x^{\mu}\}$. If the signature of the manifold is lorentzian and the 
curve time-like this affine parameter is the proper time $\tau$, and 
eq.(\ref{c2.3}) is the equation of motion of a test particle of arbitrary 
non-vanishing mass, in a fixed space-time with affine connection 
$\Gam_{\kg\nu}^{\:\:\:\:\:\mu}(x)$. Note also that the choice of 
$d\lb = ds$ implies an identity 

\be
g_{\mu\nu} \frac{dx^{\mu}}{ds} \frac{dx^{\nu}}{ds}\, =\, \pm 1,
\label{c2.4}
\ee

\nit
where again the plus sign holds for euclidean or space-like lorentzian 
curves, and the minus sign for time-like curves in lorentzian space-times.
This is a constraint on the solutions of the geodesic equation 
(\ref{c2.3}).

That this constraint is consistent with the geodesic equation follows by 
observing that

\be
H(s)\, =\, 
       \frac{1}{2}\, g_{\mu\nu} \frac{dx^{\mu}}{ds} \frac{dx^{\nu}}{ds}
\label{c2.5}
\ee

\nit
is a constant of motion, or more generally a constant of geodesic flow:

\be
\frac{dH}{ds}\, =\, g_{\mu\nu} \frac{dx^{\mu}}{ds}\, \left( 
  \frac{d^2 x^{\nu}}{ds^2} + \Gam_{\lb\kg}^{\:\:\:\:\:\nu} 
  \frac{dx^{\lb}}{ds} \frac{dx^{\kg}}{ds} \right)\,
  =\, 0. 
\label{c2.6}
\ee
  
\nit
Finally light-like curves (also called null-curves) by definition obey

\be
g_{\mu\nu} \frac{dx^{\mu}}{d\lb} \frac{dx^{\nu}}{d\lb}\, =\, 0.
\label{c2.7}
\ee

\nit
In this case the affine parameter $\lb$ can not be identified with proper 
time or distance. As eq.(\ref{c2.7}) is to hold on all points of the 
light-like curve, the quantity

\be
H(\lb)\, =\, \frac{1}{2}\, g_{\mu\nu} \frac{dx^{\mu}}{d\lb} 
             \frac{dx^{\nu}}{d\lb} = 0
\label{c2.8}
\ee

\nit
must be a constant of light-like motion. Therefore eq.(\ref{c2.6}) still
holds with $s$ replaced by $\lb$. From this it follows that it is correct
to interpret the solutions of the geodesic equation 

\be 
\frac{d^2 x^{\mu}}{d\lb^2}\, +\, \Gam_{\kg\nu}^{\:\:\:\:\:\mu} 
  \frac{d x^{\nu}}{d\lb} \frac{d x^{\kg}}{d\lb}\, =\, 0,
\label{c2.9} 
\ee 

\nit
satisfying the constraint $H(\lb) = 0$ as light-like geodesics. 
\vs

\nit
{\em Remark.}  Although we have shown that the geodesic equation implies 
the constancy of $H(\lb)$ for all types of geodesics, the inverse 
statement is not true. In particular, for  non-null geodesics (euclidean, 
and space-like or time-like lorentzian) the more general condition

\be
\frac{d^2 x^{\mu}}{d\lb^2}\, +\, \Gam_{\kg\nu}^{\:\:\:\:\:\mu} 
  \frac{d x^{\nu}}{d\lb} \frac{d x^{\kg}}{d\lb}\, =\, 
  B^{\:\mu}_{\:\:\:\nu}(x) \frac{dx^{\nu}}{d\lb} ,
\label{c2.10} 
\ee 

\nit
with $B_{\mu\nu} = - B_{\nu\mu}$ an anti-symmetric tensor, is sufficient 
for $H$ to be conserved. This happens for example for charged particles 
in an electro-magnetic field with field strength $F_{\mu\nu}$:

\be
B_{\mu\nu}(x)\, =\, \frac{q}{m}\, F_{\mu\nu}(x),
\label{c2.11}
\ee

\nit 
where $q/m$ is the charge-to-mass ratio of the particle.  Similar 
extensions exists for particles with spin or non-abelian charges. 

For light-like geodesics the equation can be further generalized to read 

\be
\frac{d^2 x^{\mu}}{d\lb^2}\, +\, \Gam_{\kg\nu}^{\:\:\:\:\:\mu} 
     \frac{d x^{\nu}}{d\lb} \frac{d x^{\kg}}{d\lb}\, =\,  
     B^{\:\mu}_{\:\:\:\nu}(x) \frac{dx^{\nu}}{d\lb} \, +\, \kg 
     \frac{dx^{\mu}}{d\lb}, 
\label{c2.12}
\ee

\nit
with $\kg$ an arbitrary constant.  It should be noted that if $\kg \neq 0$, 
then $H$ is only conserved by  virtue of the fact that it vanishes. 
\vs

\nit
{\bf Summary} \nl
The results of this discussion an be summarized as follows. All geodesic 
curves, in euclidean or lorentzian manifolds, satisfy the equation 

\be
\frac{d^2 x^{\mu}}{d\lb^2}\, +\, \Gam_{\kg\nu}^{\:\:\:\:\:\mu} 
  \frac{d x^{\nu}}{d\lb} \frac{d x^{\kg}}{d\lb}\, =\, 0,
\label{c2.13}
\ee

\nit
where $\lb$ is an affine parameter. The quantity 

\be
 H(\lb)\, =\, \frac{1}{2}\, g_{\mu\nu} \frac{dx^{\mu}}{d\lb} 
             \frac{dx^{\nu}}{d\lb} , 
\label{c2.14}
\ee

\nit 
is conserved by the geodesic flow.  In physical applications three cases 
are to be distinguished:

\begin{enumerate}
\item {For  euclidean manifolds and space-like geodesics of lorentzian 
manifolds one can take $d\lb = ds$, the proper distance; these geodesics 
are then characterized by the condition $ 2H(s) = 1$.}
\item {Time-like geodesics of lorentzian manifolds can be parametrized by 
 the proper time: $d\lb = d\tau$; such geodesics satisfy  $2H(\tau) = -1$.}
\item  {Light-like (null) geodesics admit no such identification of $\lb$ 
with invariant measures of  the arc length in an inertial frame 
(`laboratory frame'); null-geodesics are characterized  by $H(\lb) = 0$.}  
\end{enumerate} 
 

\section{Canonical formulation \label{S2.2}}

In $D$-dimensional space-time eq.(\ref{c2.13}) represents a set of $D$
second order differential equations in the affine parameter $\lb$ 
providing a covariant description of geodesics. It is possible to replace 
this set by a set of $2D$ first order differential equations by going over 
to the canonical formulation of the dynamics of test particles, in which 
the number of independent variables is doubled. Introducing the momentum 
variables 

\be
p_{\mu}(\lb) = g_{\mu\nu}(x) \frac{dx^{\nu}}{d\lb},
\label{c2.15}
\ee

\nit
the geodesic equation (\ref{c2.13}) becomes

\be
\frac{dp_{\mu}}{d\lb}\, =\, \Gam_{\mu}^{\:\:\lb\nu} p_{\lb} p_{\nu}. 
\label{c2.16}
\ee

\nit
The equations (\ref{c2.15}) and (\ref{c2.16}) constitute a pair
of first-order differential equations equivalent to the second order
geodesic equation (\ref{c2.13}). A powerful result is now obtained by 
observing that these two equations can be derived from the constant 
of motion $H(\lb)$, eq.(\ref{c2.14}) as a pair of canonical 
hamiltonian equations with $H(\lb)$ in the role of hamiltonian: 

\be
H(\lb) = \frac{1}{2}\, g^{\mu\nu} p_{\mu} p_{\nu}.
\label{c2.17}
\ee

\nit
With this definition 

\be
\frac{dx^{\mu}}{d\lb} = \dd{H}{p_{\mu}}, \hspace{3em} 
\frac{dp_{\mu}}{d\lb} = - \dd{H}{x^{\mu}}.
\label{c2.18}
\ee

\nit
Then any function $F(x^{\mu}, p_{\mu})$ on the $2D$-dimensional phase 
space spanned by the coordinates and momenta changes along a geodesic 
according to 

\be
\frac{dF}{d\lb}\, =\, \frac{dx^{\mu}}{d\lb}\, \dd{F}{x^{\mu}}\, +\, 
      \frac{dp_{\mu}}{d\lb}\, \dd{F}{p_{\mu}}\, =\, \left\{ F, H \right\},
\label{c2.19}
\ee

\nit
where the Poisson bracket of two functions $(F, G)$ on the phase space 
is defined generally as 

\be
\left\{ F, G \right\}\, =\, - \left\{ G, F \right\}\, =\, 
  \dd{F}{x^{\mu}} \dd{G}{p_{\mu}}\, -\, \dd{F}{p_{\mu}} \dd{G}{x^{\mu}}.
\label{c2.20}
\ee

\nit
The anti-symmetry of the Poisson bracket automatically guarantees
the conservation of the hamiltonian $H$ by

\be
\left\{ H, H \right\}\, =\, 0. 
\label{c2.21}
\ee

\nit
A similar property holds for all quantities which are constant 
along geodesics:

\be
\frac{dF}{d\lb} = 0 \hspace{2em} \Leftrightarrow \hspace{2em} 
\left\{ F, H \right\} = 0.
\label{c2.22}
\ee

\nit
Formal properties of the Poisson bracket include its anti-symmetry and 
its linearity in each of the arguments: 

\be
\left\{ F, \ag_1 G_1 + \ag_2 G_2 \right\} = 
  \ag_1 \left\{ F, G_1 \right\} + \ag_2 \left\{ F, G_2 \right\}.
\label{c2.23}
\ee

\nit
Another important property is that it satisfies the Jacobi identity:

\be
\lacc F, \lacc G, K \racc \racc + \lacc G, \lacc K, F \racc \racc 
  + \lacc K, \lacc F, G \racc \racc = 0.
\label{c2.24}
\ee

\nit
This property implies, that the Poisson bracket of two constants of
geodesic flow is again a constant of geodesic flow: 
if $\{ F, H \} = 0 $ and $\{ G, H \} = 0$, then 

\be
\lacc \lacc F, G \racc, H \racc = 0.
\label{c2.25}
\ee

\nit
As $H$ is itself constant on geodesics, the above results are sufficient to
establish that the constants of geodesic flow form a Lie algebra, with the 
Poisson bracket as the Lie bracket. 

The definition of the Poisson bracket (\ref{c2.20}) is not manifestly 
covariant, and therefore at first sight it seems to destroy the 
build-in covariance of the tensor calculus of differential geometry, and 
of general relativity in particular. However, note that in our definition 
the connection (\ref{c2.2.2}) is alway symmetric in its lower indices; 
therefore we can rewrite the Poisson bracket formula as

\be
\lacc F, G \racc = \cD_{\mu} F \dd{G}{p_{\mu}} - 
                   \dd{F}{p_{\mu}} \cD_{\mu} G,
\label{c2.26}
\ee

\nit
where for scalar functions $F$ and $G$ on the phase space we define
the {\em covariant} derivative

\be
\cD_{\mu} F = \pl_{\mu} F + \Gm{\mu}{\nu}{\lb} p_{\lb} \dd{F}{p_{\nu}}.
\label{c2.27}
\ee

\nit
This equation preserves manifest covariance for scalar functions $F$ and 
$G$; for example, if $J(x,p) = J^{\mu}(x) p_{\mu}$, then 

\be
\cD_{\mu} J =  \lh \pl_{\mu} J^{\nu} + \Gm{\mu}{\lb}{\nu} J^{\lb} \rh 
     p_{\nu} = \lh D_{\mu} J \rh^{\nu} p_{\nu}.
\label{c2.28}
\ee

\nit
The manifestly covariant form of the Poisson bracket can also be extended 
to all completely symmetric tensors $T_{\mu_1...\mu_n}$ of rank $n$ by 
contracting all $n$ indices with the momentum $p_{\lb}$ to obtain the 
scalar 

\be
T(x,p) = \frac{1}{n!}\, T^{\mu_1...\mu_n}(x) p_{\mu_1}...p_{\mu_n}.
\label{c2.29}
\ee

\nit
Inserting this scalar into the covariant Poisson bracket, the bracket for 
a particular tensor component $T^{\mu_1...\mu_n}$ is obtained by taking, in 
the expression resulting on the right-hand side, the coefficient of the 
$n$-nomial in the momenta that one is interested in. For anti-symmetric 
index structures a similar result can be achieved using differential forms,
or more generally Grassmann algebras \ct{RH1,RH2,GRH}. 

\section{Action principles \label{S2.3}}

The canonical formulation of geodesic flow presented here can be cast into 
the form of a standard hamiltonian action principle. Namely, the canonical 
eqs.(\ref{c2.18}) define the critical points of the phase-space action 

\be
S = \int_1^2 d\lb \lh \dot{x} \cdot p - H(x,p) \rh.
\label{c2.30}
\ee

\nit
By using the hamilton equation 

\[
\dot{x}^{\mu} = \dd{H}{p_{\mu}}, 
\]

\nit
the momentum variable can be eliminated in favour of the velocity of 
geodesic flow, to give the lagrangian form of the action

\be
S = \int_1^2 d\lb\,  \frac{1}{2}\, g_{\mu\nu}(x) \dot{x}^{\mu} 
    \dot{x}^{\nu}.
\label{c2.31}
\ee

\nit
We observe, that this is not the action for the geodesics that we started 
from, eq.(\ref{c2.1}). In particular, it is not reparametrization 
invariant. A comparison shows, that the lagrangian in (\ref{c2.31}) is  
actually the square of $w(\lb)$ used earlier, eq.(\ref{c2.2}). Clearly, 
the critical points are therefore the same, with the possible exception of
light-like curves. Actually, the variational principle for the original 
action was not even well-defined in the case of light-like curves. 

In this section we examine somewhat more closely the relation between the 
various action principles, and in particular the role of reparametrization 
invariance. It makes clear how one can derive the lagrangian and
hamiltonian actions presented above within a unified framework. 

The key to the general formulation is to incorporate reparametrization 
invariance in an action of the type (\ref{c2.31}) \ct{BHV}. This is 
achieved by introduction of a new variable $e(\lb)$, a function of the 
affine parameter, which acts as a gauge field in one dimension for local 
reparametrizations of the worldline. More precisely, the variable $e(\lb)$
by definition transforms under reparametrizations $\lb \rightarrow 
\lb^{\prime}$ as

\be
e(\lb) \rightarrow e^{\prime}(\lb^{\prime}) = 
                   e(\lb)\, \frac{d\lb}{d\lb^{\prime}}.
\label{c2.32}
\ee

\nit
This is the transformation rule for the square root of a metric in
one dimension (on a curve), for which reason the variable $e(\lb)$ is
called the einbein. Written in a slightly different way, eq.(\ref{c2.32})
states that $e(\lb) d\lb$ is defined to be invariant under 
reparametrizations. This makes it straightforward to write a 
reparametrization-invariant form of the quadratic action (\ref{c2.31}):

\be
S[e;x] = \int_1^2 d\lb\, \lh \frac{1}{2e}\, g_{\mu\nu}(x) 
       \frac{dx^{\mu}}{d\lb} \frac{dx^{\nu}}{d\lb} - \frac{c^2}{2} e \rh.
\label{c2.33}
\ee
  
\nit
The last term, proportional to the constant $c^2$, does not depend on the 
coordinates $x^{\mu}$. However, it is reparametrization invariant and its 
inclusion is important for reasons given below. 

Variation of the full action $S[e;x]$ w.r.t.\ the coordinates $x^{\mu}$ 
reproduces the geodesic equation (\ref{c2.13}) provided everywhere the 
differentials $d\lb$ are replaced by $e d\lb$. This replacement makes 
the geodesic equation reparametrization invariant, as $e d\lb = \pr{e} 
d \pr{\lb}$. On the other hand, the substitution $e(\lb) = 1$, which 
breaks reparametrization invariance, makes the old and new equations 
fully identical. Such a substitution is allowed because it only serves 
to define the affine parameter $\lb$ in terms of quantities measurable 
by an observer in the locally euclidean or lorentzian laboratory frame, 
like proper length or proper time. Of course, such a choice necessarily 
breaks the reparametrization invariance, but it preserves the physical 
content of the equations. It amounts to a choice of gauge for 
reparametrizations in the true sense of the expression, with the result 
that modulo a constant the action $S[e;x]$ reduces to the simple 
quadratic action (\ref{c2.31}). 

However, the action $S[e;x]$ contains more information, as one can
also consider its variation w.r.t.\ the einbein $e$. Requiring stationarity
under this variation gives a constraint on the solutions of the geodesic 
equation, which after multiplication by $2e^2$ takes the form

\be
g_{\mu\nu}(x) \dot{x}^{\mu} \dot{x}^{\nu} + e^2 c^2 = 0.
\label{c2.34}
\ee

\nit
With $e = 1$, comparison with the definition of $H$ in eq.(\ref{c2.5}) shows 
that this constraint expresses the constancy of the hamiltonian along a
geodesic:

\be
2H(\lb) = - c^2.
\label{c2.35}
\ee

\nit
For euclidean manifolds one can always choose units such that $c^2 = -1$, 
but for lorentzian space-times $c^2 = (-1, 0, +1)$ corresponds to 
space-like, light-like or time-like geodesics respectively; in the
latter case the constant $c$ then represents the speed of light, which
is unity when expressed in natural units. 

Finally we derive the original reparametrization-invariant geodesic action 
(\ref{c2.1}) from $S[e;x]$. This is achieved by using eq.(\ref{c2.34})
to solve for $e$, instead of fixing a gauge: 
\
\be
e = \pm \sqrt{\left| g_{\mu\nu} \dot{x}^{\mu} \dot{x}^{\nu}/c^2 \right|}.
\label{c2.37}
\ee

\nit
Substitution of this expression for $e$ into the action $S[e;x]$ then
leads back (modulo a possible sign) to the original action (\ref{c2.1}).
Therefore we conclude that both this action and the quadratic action
(\ref{c2.31}) follow from the same starting point provided by 
eq.(\ref{c2.33}). 

\section{Symmetries and Killing vectors \label{S2.4}}
   
Often space-times of interest possess special symmetries. Such symmetries 
are useful in finding solutions of the geodesic equations, especially if 
they are continuous symmetries as these generate constants of geodesic flow.
 This is the content of Noether's theorem applied to the motion of test 
particles and its generalization to space-like curves; see for example 
refs.\ct{MTW}-\ct{KSMH}, \ct{RH1,RH2}. In this section the role of 
continuous symmetries is explored in some detail. 

A manifold possesses a continuous symmetry, or isometry, if there are 
infinitesimal coordinate transformations leaving the metric invariant. 
Finite transformations can be obtained by reiteration of the infinitesimal 
transformations, and donot require separate discussion at this point. 
Consider an infinitesimal coordinate transformation characterised by local 
parameters $\xi^{\mu}(x)$: 

\be
x^{\mu}\, \rightarrow\, x^{\prime\, \mu} = x^{\mu} - \xi^{\mu}(x) .
\label{c2.38}
\ee

\nit
For the line element $ds^2$ to be invariant the metric must transform as a 
tensor; therefore by definition 

\be
g_{\mu\nu}(x) = g^{\prime}_{\kg\lb}(x^{\prime}) 
 \dd{x^{\prime\, \kg}}{x^{\mu}} \dd{x^{\prime\, \lb}}{x^{\nu}}.
\label{c2.40}
\ee

\nit
On the other hand, invariance of the metric under a coordinate 
transformation implies 

\be 
g^{\prime}_{\mu\nu}(x) = g_{\mu\nu}(x).
\label{c2.39}
\ee

\nit
Combining the two equations (\ref{c2.40}) and (\ref{c2.39}) to eliminate 
the transformed metric $g^{\prime}_{\mu\nu}$, and inserting the 
infinitesimal transformation (\ref{c2.38}), expansion to first order in 
$\xi^{\mu}$ leads to the covariant condition 

\be
D_{\mu} \xi_{\nu} + D_{\nu} \xi_{\mu} = 0.
\label{c2.41}
\ee

\nit
This equation is known as the Killing equation, and the vector fields 
defined by the solutions $\xi^{\mu}(x)$ are called Killing vectors. The 
existence of a Killing vector is equivalent with the existence of an 
infinitesimal coordinate transformation (\ref{c2.38}) leaving the metric 
invariant. 

Let us pause for a moment to reflect on the interpretation of this result. 
If the coordinate transformation is considered to be a passive 
transformation, the new coordinates represent a relabeling of the points of 
the manifold: $x^{\mu}$ and $x^{\prime\, \mu}$ in eq.(\ref{c2.38}) refer to 
the same point $\cP$. Now consider the point $\pr{\cP}$, which in the new 
coordinate system has the same value of the coordinates as the point $\cP$ 
in the old coordinate system: $x^{\prime\, \mu}(\pr{\cP}) = x^{\mu}(\cP)$. 
Eq.(\ref{c2.39}) states that the new metric at the point $\pr{\cP}$ has 
the same functional dependence on the new coordinates as the old metric on 
the old coordinates at the point $\cP$. Thus in the new coordinate system 
the neighborhood of $\pr{\cP}$ looks identical to the neighborhood of $\cP$ 
in the old coordinates. In particular it is possible to map the points in 
the neighborhood of $\cP$ one-to-one to points in the neighborhood of 
$\pr{\cP}$ in such a way that all distances (intervals) are preserved. As 
this is in fact a coordinate-invariant statement, it implies a local 
indistinguishability of the two neighborhoods of the manifold (as long as 
it is not endowed with additional structures). This then is what is implied 
by a continuous symmetry of the manifold generated by the solutions of the 
Killing equation.

Now if two neighborhoods of the manifold are similar in the sense described 
above, then this similarity should also extend to the geodesics passing 
through the points mapped on each other by the symmetry operation. Indeed, 
as the new metric at the point $\pr{\cP}$ has the same {\em functional 
dependence} on the new coordinates there as the old metric at $\cP$ has on 
the old coordinates, and not just the same value, the connections and 
curvature components there also become identical after the coordinate 
transformation. The same holds for the solutions of the geodesic 
equations. Thus the symmetry transformation maps geodesics through the 
point $\cP$ to geodesics through the point $\pr{\cP}$, and the geodesic 
flow in the neighborhood of these points is completely similar. 
\vs

\nit
The similarity of geodesic structure generated by symmetry operations 
implies the conservation of certain dynamical quantities under geodesic 
flow. This is most conveniently discussed in the canonical formalism of the 
geodesic flow presented above in sect.\ref{S2.2}. The quantity conserved is 
the generator of the symmetry transformations, obtained by contraction of 
the Killing vector with the canonical momentum:

\be
J[\xi] = \xi^{\mu}(x) p_{\mu}.
\label{c2.42}
\ee

\nit
This is a scalar quantity, hence its value is coordinate invariant. It 
generates the infinitesimal coordinate transformations through the Poisson 
bracket (\ref{c2.20}):

\be
\del x^{\mu} = - \xi^{\mu}(x) = \lacc J[\xi], x^{\mu} \racc. 
\label{c2.43}
\ee

\nit
One can similarly determine the variation of the momentum under the 
transformation generated by $J[\xi]$:

\be
\ba{lll}
\del p_{\mu} & = & \lacc J[\xi], p_{\mu} \racc \\
 & & \\
 & = & \pl_{\mu} J[\xi]\, =\, T_{\mu}^{\;\:\nu}(x) p_{\nu}
\ea
\label{c2.44}
\ee

\nit
with $T_{\mu}^{\;\:\nu} = \pl_{\mu} \xi^{\nu}$. This represents a 
coordinate-dependent linear transformation of the momentum. 

That the quantity $J[\xi]$ is conserved now follows from the observation 
that the hamiltonian is invariant under the phase-space transformations 
defined in eqs.(\ref{c2.43}), (\ref{c2.44}). Indeed, taking into account 
the canonical equations of motion (\ref{c2.19}) and (\ref{c2.22}), and 
using the Killing equation (\ref{c2.41}) we obtain 

\be
\frac{dJ[\xi]}{d\lb}\, =\, \lacc J[\xi], H \racc\, =\, 0.
\label{c2.45}
\ee

\nit
This result was to be expected, as the hamiltonian depends on the 
coordinates only through the metric, which is invariant by definition of an 
isometry. 
\vs

\nit
As the Killing equation (\ref{c2.41}) is linear it follows that the Killing 
vectors define a linear vector space: any linear combination of two Killing 
vectors is again a Killing vector. Let the dimension of this vector space 
be $r$; then any Killing vector can be expanded in terms of $r$ linearly 
independent basis vectors $e_i(x)$, $i = 1,...,r$:

\be
\xi(\ag_i) = \ag_1 e_1(x) + ... + \ag_r e_r(x).
\label{c2.46}
\ee

\nit
Equivalently, any infinitesimal symmetry transformation (\ref{c2.38}) 
depends linearly on $r$ parameters $\ag_i$, to which correspond an equal 
number of conserved generators 

\be
J[\xi] = \ag_1 J_1 + ... + \ag_r J_r, \hspace{3em} \mbox{where} \hspace{1em}
    J_i(x,p) = e_i^{\mu}(x) p_{\mu}.
\label{c2.47}
\ee

\nit
We now show that these generators define a Lie algebra through their Poisson
brackets. The key observation is, that the Poisson bracket of any two 
constants of geodesic flow is itself a constant of geodesic flow. This is 
implied by the Jacobi identity for the Poisson bracket, which can be 
written as:

\be
\lacc \lacc F, G \racc, H \racc\, =\, \lacc \lacc F, H \racc, G \racc
\, -\, \lacc  \lacc G, H \racc, F \racc.
\label{c2.48}
\ee

\nit
Thus, if the Poisson brackets of $F$ and $G$ with the hamiltonian $H$ 
vanish, then the left-hand side vanishes as well, and $\lacc F, G \racc$ is 
itself a constant of geodesic flow. 

A second important observation is, that for two constants of motion which 
are linear in the momentum, like the $J_i$, the Poisson bracket is also 
linear in the momentum:

\be
\lacc J_i, J_j \racc\, =\, \lh e_j^{\nu} \pl_{\nu} e_i^{\mu} -  
   e_i^{\nu} \pl_{\nu} e_j^{\mu} \rh\, p_{\mu}.
\label{c2.49}
\ee

\nit
As the $\lacc J_i \racc_{i=1}^{r}$ are supposed to form a complete set, the
expression on the right-hand side can be expanded in terms of the basis 
elements, with the result that with a certain set of coefficients 
$f_{ij}^{\:\:\:\:k} = - f_{ji}^{\:\:\:\:k}$ we have 

\be
\lacc J_i, J_j \racc\, =\, f_{ij}^{\:\:\:\:k}\, J_k.
\label{c2.50}
\ee

\nit
An equivalent statement is that the basis vectors of the Killing space 
satisfy 

\be 
 e_j^{\nu} \pl_{\nu} e_i^{\mu} - e_i^{\nu} \pl_{\nu} e_j^{\mu}\, =\, 
   f_{ij}^{\:\:\:\:k}\, e_k^{\mu}.
\label{c2.51}
\ee

\nit
Eq.(\ref{c2.50}), combined with the observations that the $J_i$ form a 
linear vector space and that the Poisson bracket is bilinear and 
anti-symmetric in its arguments complete the proof that the generators 
of the symmetry transformations define a Lie algebra with structure 
constants $f_{ij}^{\:\:\:\:k}$. 

Of course the linear p.d.e.(\ref{c2.51}) encodes the same information. It 
can be interpreted in terms of the Lie-derivative, which is the operator 
comparing the value of a function at the point $\cP$ with that at the point 
$\pr{\cP}$ which has the same value of its coordinates after an arbitrary 
transformation of the form (\ref{c2.38}) as the point $\cP$ had before the 
transformation: $x^{\prime\, \mu} (\pr{\cP}) = x^{\mu} (\cP)$. For a scalar 
$\fg(x)$, for which $\pr{\fg}(\pr{x}) = \fg(x)$, this gives 

\be
\cL_{\xi}\left[ \fg \right](x)\, \equiv\, \mbox{lin}_{\xi} 
  \left[ \pr{\fg}(x) - \fg(x)\right]\, =\, \xi^{\nu} \pl_{\nu} \fg(x),
\label{c2.52}
\ee

\nit
where the lin$_{\xi} [Q]$ denotes the part of the expression $Q$ linear in 
$\xi$. For a vector $v^{\mu}(x)$, for which 

\be
v^{\prime\, \mu} (\pr{x})\, =\,  v^{\nu}(x) \dd{x^{\prime\, \mu}}{x^{\nu}},
\label{c2.53}
\ee

\nit
one finds similarly 

\be
\lh \cL_{\xi}\left[ v \right] \rh^{\mu}(x)\, \equiv\, \mbox{lin}_{\xi} 
 \left[ v^{\prime\, \mu}(x) - v^{\mu}(x) \right]\, =\, 
  \xi^{\nu} \pl_{\nu} v^{\mu}(x) - \pl_{\nu} \xi^{\mu} v^{\nu}(x).
\label{c2.54}
\ee

\nit
For higher-rank tensors the construction of the Lie-derivative gives the 
result 

\be 
\ba{lll}
\lh \cL_{\xi}\left[ T \right] \rh^{\mu_1...\mu_k}(x) & \equiv & 
  \mbox{lin}_{\xi} \left[ T^{\prime\, \mu_1...\mu_k}(x) - 
  T^{\mu_1...\mu_k}(x) \right] \\
 & & \\
 & = &  \xi^{\nu} \pl_{\nu} T^{\mu_1...\mu_k}(x) - \pl_{\nu} \xi^{\mu_1} 
     T^{\nu...\mu_k}(x) - ... - \pl_{\nu} \xi^{\mu_k} T^{\mu_1...\nu}(x). 
\ea
\label{c2.54.1}
\ee

\nit
Now comparing eqs.(\ref{c2.51}) and (\ref{c2.54}) we see that the Lie-algebra 
property of the Killing vectors may be expressed as 

\be
\cL_{e_j}[e_i]\, =\, - \cL_{e_i}[e_j]\, =\, f_{ij}^{\;\;\;\;k}\, e_k.
\label{c2.55}
\ee

\nit
Finally, in the phase space where by definition $\pl_{\nu} p_{\mu} = 0$, 
we can also write the transformation (\ref{c2.44}) for the momentum as 

\be
\del_i p_{\mu} \equiv \lacc J_i, p_{\mu} \racc\, =\, \lh \cL_{e_i}[p] 
   \rh_{\mu}.
\label{c2.56}
\ee

\nit
Thus we have established a close relationship between Poisson brackets
and Lie derivatives, and between symmetries, Killing vectors and Lie 
algebras. 

\section{Phase-space symmetries and conservation laws \label{S2.5}}

In the previous section it was established that continuous symmetries of 
manifolds are generated by Killing vectors and imply conservation laws for 
certain dynamical quantities (the generators $J$) along geodesics. However, 
not every constant of geodesic flow is necessarily connected with a Killing
vector. This is most easily seen from the example of the hamiltonian itself,
which is conserved but not of the form (\ref{c2.42}). Rather the hamiltonian
is quadratic in the momenta. This leads us to consider the possibility of 
conservation laws for quantities which are higher order expressions in the 
momenta. 

Let $J(x,p)$ be any function on the phase space of coordinates 
$x^{\mu}(\lb)$ and momenta $p_{\mu}(\lb)$, associated with a geodesic, 
which is non-singular in the momenta. In others words, we suppose it has an 
expansion of the type

\be
J(x,p) = \sum_{k=0}^{\infty}\, \frac{1}{k!}\, J^{(k)\, \mu_1...\mu_k}(x)\, 
         p_{\mu_1}...p_{\mu_k}.
\label{c2.57}
\ee

\nit 
Here the coefficients $J^{(k)}$ can be taken to be completely symmetric in 
all $k$ indices. We ask under what conditions such a function can be a 
constant of geodesic flow:

\be
\frac{dJ}{d\lb}\, =\, \lacc J, H \racc\, =\, 0.
\label{c2.58}
\ee

\nit
To obtain the answer, insert the expansion (\ref{c2.57}) into this equation 
and compare terms at equal order of powers of momentum.  At zeroth order one 
finds 

\be
\pl_{\mu} J^{(0)} = 0,
\label{c2.58.1}
\ee

\nit
i.e.\ $J^{(0)}$ is a constant. Such a constant can always be absorbed in 
the definition of $J$ and is of no consequence. From now on it will be 
dropped.

At first order one finds back the Killing equation (\ref{c2.41}):

\[
D_{\mu} J^{(1)}_{\nu} + D_{\nu} J^{(1)}_{\mu} = 0.
\]

\nit
These terms we have already discussed in detail. 

Finally, for $k \geq 2$ we find a generalization of the Killing equation 
for the co-efficients $J^{(k)\, \mu_1...\mu_k}(x)$:

\be
D_{\lh \mu_1 \rd} J^{(k)}_{\ld \mu_2...\mu_{k+1} \rh}\, =\, 0.
\label{c2.59}
\ee

\nit
The parentheses denote full symmetrization over all component indices 
enclosed. The solutions of these generalised Killing equations are called 
Killing tensors. It is now obvious that the hamiltonian is included, 
because the metric $g_{\mu\nu}$ is covariantly constant, and therefore 
automatically a solution of eq.(\ref{c2.59}) for $k = 2$. Moreover, this 
solution always exists, independent of the particular manifold considered. 
In addition, for specific manifolds (specific metrics $g_{\mu\nu}$) other 
solutions may exist as well. For example, in spherically symmetric spaces 
the square of the angular momentum:

\be
L^{2} = \frac{1}{2}\, \lh x^2 p^2 - \lh x \cdot p \rh^2 \rh, 
\label{c2.60}
\ee

\nit
is conserved and quadratic in the momenta by construction. Other examples 
will be encountered later on. 

Just as the Killing vectors, the Killing tensors generate symmetry 
transformations, not of the manifold but rather of the corresponding phase 
space spanned by the coordinates and the momenta (tangent vectors). In
particular:

\be
\del x^{\mu}\, =\, \lacc J(x,p), x^{\mu} \racc\, =\, -\, J^{(1)\, \mu}(x)\, 
   -\, \sum_{k=2}^{\infty}\, \frac{1}{(k-1)!}\, 
   J^{(k)\, \mu \mu_2...\mu_k}(x) p_{\mu_2}...p_{\mu_k}.
\label{c2.60.1}
\ee

\nit
We observe that the transformations generated by the higher-order Killing 
tensors are velocity dependent \ct{RH1}. 

Finally we address the algebraic properties of the constants of geodesic 
flow. We have already remarked, that the Poisson brackets of two such 
constants yields another constant by the Jacobi identity (\ref{c2.48}). In 
general the rank of quantities on the left-hand side are additive minus one:

\be
\lacc J^{(k)}, J^{(l)} \racc\, \sim J^{(k+l-1)}.
\label{c2.61}
\ee

\nit
Now for $l = 1$ the rank of $J^{(k+l-1)}$ is the same as that 
of $J^{(k)}$. It follows, that \nl 
$(i)$ for the constants of geodesic flow linear in the momentum, 
corresponding to Killing vectors $(k = l = 1)$, the algebra is closed in 
itself: it is a Lie-algebra $G$; \nl
$(ii)$ for any fixed value of $k$, the brackets of a $J^{(1)}$ and a 
$J^{(k)}$ close on the $J^{(k)}$; however, the brackets of two elements 
$J^{(k)}$ generates an element of order $(2k-1)$. Hence in general the 
algebra (\ref{c2.61}) is not closed, unless one includes elements of 
arbitrary rank, i.e.\ all possible $k$. This implies that once higher-order
invariants appear, one may expect an infinite series of them. 
Sometimes this happens indeed, as with the Virasoro algebra for the 
conformal transformation in two dimensions \ct{GSW}. However, in many cases 
the series stops because the higher order invariants are Casimir-type of 
operators, or they become trivial in that they are just products of 
commuting lower-order elements (commuting here is meant in the sense of 
vanishing Poisson brackets). 

The Lie algebra $G$ of Killing vectors is characterized by its structure 
constants $f_{ij}^{\;\;\;\;k}$. As the Poisson brackets of $J^{(k)}$ with 
all elements of the Lie algebra spanned by the $J^{(1)}$ are again of order 
$k$, one may choose a basis $\lacc e_A^{(k) \mu_1...\mu_k}(x) \racc$ for 
the Killing tensors of order $k$, labeled by the index $A$, and decompose 
the right-hand side of the Poisson bracket again in terms of the 
corresponding conserved charges $J_A^{(k)}$:
 
\be
\lacc J_i^{(1)}, J_A^{(k)} \racc\, =\, g_{iA}^{\;\;\;\;B}\, J_B^{(k)}.
\label{c2.62}
\ee

\nit
This defines a set of higher-order structure constants. The Jacobi 
identities then imply, that the matrices $(T_i)_A^{\;\;B} = - 
g_{iA}^{\;\;\;\;B}$ define a representation of the Lie algebra 
(\ref{c2.50}):

\be
g_{jA}^{\;\;\;\;C} g_{iC}^{\;\;\;\;B} - g_{iA}^{\;\;\;\;C} 
    g_{jC}^{\;\;\;\;B} = f_{ij}^{\;\;\;\;k}\, g_{kA}^{\;\;\;\;B} 
   \hspace{2em} \Longleftrightarrow  \hspace{2em} 
\left[ T_i, T_j \right]_{A}^{\;\;B}\, =\, f_{ij}^{\;\;\;\;k}\, 
  T_{kA}^{\;\;B}.
\label{c2.63}
\ee

\nit
Therefore the constants of geodesic flow 

\be
J_A^{(k)}\lh x, p\rh\, =\, \frac{1}{k!}\, e_A^{(k) \mu_1...\mu_k}(x) 
    p_{\mu_1} ...p_{\mu_k},
\label{c2.64}
\ee

\nit
span a representation space of the Lie algebra $G$ for the representation 
$\lacc T_i \racc$. The discussion of symmetries shows that group theory 
and Lie algebras can be important tools in the analysis of geodesic motion 
and the structure of manifolds.  

\section{Example: the rigid rotor \label{S2.6}}

The above concepts and procedures can be illustrated by the simple example 
of a rigid rotor, which has a physical interpretation as a model for the 
low-energy behaviour of diatomic molecules. As such the example also 
serves to emphasize the usefulness of geometric methods in physics outside 
the context of general relativity. 

Consider two particles of mass $m_1$ and $m_2$, interacting through a central 
potential $V(r)$ depending only on the relative distance $r = 
\left|{\br_2} - {\br_1}\right|$. The lagrangian for this system is

\be
L\, =\, \frac{m_1}{2}\, { \dot{\br}_1}^2\, +\, \frac{m_2}{2}\, 
  { \dot{\br}_2}^2\, -\, V(r).
\label{c2.65}
\ee

\nit
Defining as usual the total mass $M = m_1 + m_2$ and the reduced mass
$\mu = m_1 m_2/M$, the lagrangian is separable in the center of mass 
coordinates defined by

\be
M {\bR}\, =\, m_1 {\br_1}\, +\, m_2 {\br_2}, \hspace{3em}
{\br}\, =\, {\br_2}\, -\, {\br_1}.
\label{c2.66}
\ee

\nit
In terms of $({\bR}, {\br})$ the expression (\ref{c2.65}) becomes

\be
L\, =\,
 \frac{M}{2}\, { \dot{\bR}}^2\, +\, \frac{\mu}{2}\, { \dot{\br}}^2\,
 -\, V(r).
\ee

\nit
As the center of mass moves like a free particle of mass $M$, it is 
convenient to work in the rest frame of the center of mass: ${\bR} = 0$. 
Then we are only left with the problem of describing the relative motion of 
the masses, described by the three coordinates represented by the vector 
${\br}$.  

Now suppose that the potential $V(r)$ has a minimum for some 
separation $ r = r_0 $, and rises steeply for all values of $ r $  
near this minimum. Then the first excited vibration state of the molecule 
has an energy well above the ground state, and at low temperatures the only 
degrees of freedom that play a role in the dynamics are rotations of the 
molecule at fixed interatomic distance $r_0$. Thus the distance is frozen 
out as one of the dynamical degrees of freedom, and we are effectively 
left with only two coordinates: the angles $(\th, \vf)$ describing the 
relative orientation of the two masses; the potential $V(r) = V(r_0)$ is constant and may be ignored. This leaves as the effective action of the 
system

\be
L_{eff}\, =\, \frac{\mu}{2}\, r_0^2\, \lh \dot{\th}^2 + \sin^2 \th\, 
  \dot{\vf}^2 \rh.
\label{c2.67}
\ee 

\nit
This is the lagrangian of a particle of mass $\mu$ moving on a spherical
surface of radius $r_0$. In mathematical physicists' parlance the effective 
low energy degrees of freedom $(\th, \vf)$ are sometimes called the modular 
parameters or moduli of the system, and the sphere representing the effective 
low-energy configuration space is called the moduli space. 

Up to an overall scale factor $\mu r_0^2$, the lagrangian $L_{eff}$ represents 
an action of the form (\ref{c2.31}) in a 2-dimensional space with euclidean 
signature, described by the coordinates $x^1 = \th$, $x^2 = \vf$ and metric 

\be
g_{ij}\, =\, \lh \ba{cc} 
                 1 & 0 \\
                 0 & \sin^2 \th \ea \rh.
\label{c2.68}
\ee

\nit
As the geodesics on a sphere are great circles, the great circles provide
the general solution to the equations of motion. The spherical symmetry 
implies that the system is invariant under 3-dimensional rotations
(rotations about each of three independent body axes of the sphere) and 
hence there are three Killing vectors generating these rotations. The
corresponding constants of motion are the 3 components of angular momentum
${\bL} = ( L_1,  L_2,  L_3)$, given explicitly by 

\be
\ba{l}
L_1\, = \, \dsp{ 
          -\sin \vf\, p_{\th}\, -\, \cot \th \cos \vf\, p_{\vf}, }\\ 
  \\
L_2\, =\, \dsp{ 
          \cos \vf\, p_{\th}\, -\, \cot \th \sin \vf\, p_{\vf}, }\\
  \\
L_3\, =\, \dsp{ p_{\vf}. }       
\ea
\label{2.68.1}
\ee

\nit
They span the Lie-algebra so(3) of 
the 3-dimensional rotation group:

\be
\lacc L_i, L_j \racc\, =\, \ve_{ijk}\, L_k.
\ee

\nit
As the Poisson brackets of ${\bL}$ with the hamiltonian vanish, the hamiltonian can depend only on the Casimir constant of the rotation group, 
i.e.\ the total angular momentum squared ${\bL}^2$. A direct computation 
shows, that up to the constant potential the effective hamiltonian is in 
fact proportional to the Casimir invariant:

\be
H_{eff}\, =\,  \frac{{\bL}^2}{2 \mu r_0^2}.
\label{c2.69}
\ee

%\nit
%{\bf Exercise} \vs
%
%\nit
%\begin{enumerate}
%\item Compute explicit expressions for the canonical momenta and the 
%hamiltonian of the system defined by $L_{eff}$ in eq.(\ref{c2.67}).  
%\item Compute the connections $\Gm{i}{j}{k}$ for the metric $g_{ij}$ in
%eq.(\ref{c2.68}). Write down the equation for the Killing vectors, and 
%give the general solution. Show that the solutions generate 3-dimensional 
%rotations and define the components of angular momentum. 
%\item Show that the hamiltonian is proportional to the total angular 
%momentum squared as in eq.(\ref{c2.69}).
%\end{enumerate}



